Impact of LLM-based Review Comment Generation in Practice: A Mixed Open-/Closed-source User Study

We conduct a large-scale empirical user study in a live setup to evaluate the acceptance of LLM-generated comments and their impact on the review process. This user study was performed in two organizations, Mozilla (which has its codebase available as open source) and Ubisoft (fully closed-source). Inside their usual review environment, participants were given access to RevMate, an LLM-based assistive tool suggesting generated review comments using an off-the-shelf LLM with Retrieval Augmented Generation to provide extra code and review context, combined with LLM-as-a-Judge, to auto-evaluate the generated comments and discard irrelevant cases. Based on more than 587 patch reviews provided by RevMate, we observed that 8.1% and 7.2%, respectively, of LLM-generated comments were accepted by reviewers in each organization, while 14.6% and 20.5% other comments were still marked as valuable as review or development tips. Refactoring-related comments are more likely to be accepted than Functional comments (18.2% and 18.6% compared to 4.8% and 5.2%). The extra time spent by reviewers to inspect generated comments or edit accepted ones (36/119), yielding an overall median of 43s per patch, is reasonable. The accepted generated comments are as likely to yield future revisions of the revised patch as human-written comments (74% vs 73% at chunk-level).

==> figures/RQ1_by_user.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{img/RQ1_acceptation_by_user.pdf}
    \caption{Acceptation rate [\%] by user.\Do{display will be fixed}}
    \label{fig:RQ1_by_user_acc}
    \includegraphics[width=.9\linewidth]{img/RQ1_appreciation_by_user.pdf}
    \caption{Appreciation rate [\%] by user.\Do{display will be fixed}}
    \label{fig:RQ1_by_user_app}
\end{figure}

==> old/2-background.tex <==

\Do{Motivational example hidden here}
% \input{sections/motivation_example}

% \subsection{Background}
This section introduces the necessary concepts and terminology used in our study.

\subsubsection{Large Language Models}
A large language model (LLM) is a machine learning model trained on a vast number of parameters and owning advanced learning capabilities~\cite{chang2023survey}. 
These models usually require large training datasets, including diverse data types, like textual, image, audio, and structured data.
As a result, we can observe LLMs for different purposes, including commercial, academic, and open-source models \cite{li2023starcoder, feng2020codebert,touvron2023llama}.
Over time, LLMs trained on textual data brought the attention of users, scientists, and maintainers due to their capabilities of performing natural language processing (NLP) tasks~\cite{chowdhary2020natural}.
Specifically, in Software Engineering, LLMs have been applied in diverse tasks supporting human-like text generation \cite{xu2022systematic, fan2023large}.
For example, LLMS can be adopted for performing tasks aiming to speed up the developer's productivity, like refactoring~\cite{shirafuji2023refactoring}, testing~\cite{schafer2023empirical}, and commit messaging~\cite{zhang2024using}.
%With millions to billions of parameters, LLMs are used for various natural language processing tasks.

Considering the current popularity of LLMs, ChatGPT, a language model developed by OpenAI, stands out as one of the most popular. 
The LLM is built on GPT architecture, and it has been used for a variety of applications, among which we may highlight code generation, summarization, translation, testing, and documentation \citep{zheng2023towards, ozkaya2023application}.
OpenAI offers different models, considering active and deprecated ones.
All models are available online through an API, facilitating the process of prompting the models and escalating the number of requests.
\toolName\ adopts the variant \texttt{GPT-4o} as its base LLM; we decided to consider this version, considering its advanced capabilities compared to previous models, based on our exploratory analysis.
Further details about how we integrate and prompt the LLM are provided in Section~\ref{sec:solution}.

\subsubsection{Prompt Engineering}
To guide the LLMs in performing their tasks accurately, users rely on the prompts given as input when making requests to LLMs.
This process of defining, maintaining, and improving prompts is the study subject of Prompt Engineering, a field that combines artificial intelligence and NLP tasks~\cite{beurer2023prompting}.
When designing their prompts, users aim to create prompts based on principles like clarity and relevance~\cite{arawjo2023chainforge}.

Different approaches can be used to structure the prompts.
For example, while \emph{zero-shot} prompts rely exclusively on the instructions associated with a given specific task~\cite{radford2019language}, \emph{few-shot} approaches further support the LLM by providing a few examples and guiding the LLM about the expected behavior~\cite{nashid2023retrieval,brown2020language}. 
Regarding the reasoning of LLMs, \emph{Chain-of-Thought} plays an important role by posing a set of intermediate reasoning steps, supporting the LLM to address tasks that require complex reasoning~\cite{wei2022chain}.
Users may also play with intrinsic characteristics, like human pre-defined behavior patterns~\cite{white2023prompt}.
This way, users may require LLMs to emulate a specific persona or behavior when performing the required tasks.
\toolName\ relies on some of the previous prompting approaches, like \emph{few-shot} and \emph{chain-of-though}; further details about the way these approaches are used can be found in Section \ref{sec:solution}.

==> old/NOTUSED3-solution.tex <==



This section details the two LLM-based techniques for review comment generation's acceptance evaluated in our user study. 
First, we present the process of collecting the information associated with a contribution, including the patch under analysis. 
Next, we discuss the LLM-based techniques themselves, including the adopted prompt engineering approaches, relying on \emph{few-shot} and \emph{chain-of-though}, and Retrieval-Augmented Generation, which included in the prompt additional code and previous code changes and their associated comments which are similar changes to the target code, when available.
Then, we finally discuss the integration of the techniques into the review environments of the user study participants and how reviewers might interact with them.
The rest of this section will describe the resulting workflow, summarized in Algorithm~\ref{alg:tool-workflow}.

\input{algorithms/tool}
\input{tables/prompts}

\subsection{Starting Point}
\toolName\ is automatically called when a user opens any revision on their review tool under some constraints. 
Only revisions labeled as \emph{Needs Review} are candidates to be analyzed (line 1, Algorithm \ref{alg:tool-workflow}); at this stage, developers wait for comments to potentially submit revisions to that review. 
% For these cases, \toolName\ adds a new action in the revision scope, informing that no suggestions will be provided based on the revision status.
Next, for a given valid review, \toolName\ accesses the current patch associated with the revision and starts to analyze it. 
% First, \toolName\ computes the number of tokens associated with the given patch. 
% If the size is larger than 3000 tokens, no further actions are taken, as longer patches impact the length constraints of token limits (line 2, Algorithm~\ref{alg:tool-workflow}).
% For these cases, \toolName\ also adds a new action in the revision scope, informing that no suggestions will be provided due to the revision's size.
% Once these initial constraints are satisfied, \toolName\ moves forward with the second step of its workflow.
Review suggestions are generated once per review and kept in cache to keep consistency if reviewers reload the page. Thus, if multiple users open the same revision, they will see the same previously generated content.
% \Do{we do show the reviews to authors too} However, \toolName\ does not show the contents of a review to the revision's author.
% We believe that showing the review could bias the author to apply changes in the code that were not properly required/evaluated by another developer.

With the patch to be analyzed, \toolName\ formats the patch to highlight the ongoing changes (line 2, Algorithm \ref{alg:tool-workflow}).
Knowing that a patch consists of one or more chunks (i.e., code diff snippet), \toolName\ depicts the patch, grouping their chunks at the file level while adding the corresponding line number to the code lines.
We decided to format the chunks to filter out unnecessary information directly provided by Git while explicitly informing the context of the changed lines (addition, removal, or regular ones).
Regarding informing the numbers of the code lines, we consider an efficient way to guide the tool in associating the provided review comments with the target lines.
% \subsection{Generating Context Inputs}

% \subsubsection{Patch format}


% \subsubsection{Patch summary}
% \toolName\ performs a set of requests to the LLM under analysis.


\subsection{Retrieval-Augmented Generation}~\label{approach_sec}

\toolName\ requests the LLM to summarize the patch using the formatted patch (line 3, Algorithm \ref{alg:tool-workflow}; prompt (1) shown in Table~\ref{tab:prompts}), following state-of-the-art techniques~\cite{zheng2023take, wei2022chain}. 

We consider two ways of providing extra context for the comment generation prompt, approach "\textit{Code}" and "\textit{Example}". Although both approaches are complementary, as a first effort to evaluate the impact of generated comments on the review process, we only considered one approach at a time.

\subsubsection{Code context (\textbf{Code})}
Being aware that the patch under analysis might not have all the details to perform a good analysis, we ask the LLM whether there are function calls referred by the patch that request more context, i.e. the function declaration (line 5, Algorithm \ref{alg:tool-workflow}).
For that, we feed the patch and its associated summary to the model, yielding a list of the names of requested functions (see prompt (2) shown in Table~\ref{tab:prompts}).
For each function name, \toolName\ accesses the respective project repository and retrieves the function's declaration~\cite{ardito2020rust} (line 8, Algorithm \ref{alg:tool-workflow}).

Then, the way chunks are defined only show 10 lines of context (i.e. unmodified lines above or below modified lines). This might too lead to missing context to understand the change.
Thus, we ask the LLM whether it requires additional context for specific patch lines (line 6, Algorithm \ref{alg:tool-workflow}; prompt (3) shown in Table~\ref{tab:prompts}), this time getting extended context around the requested lines by retrieving the function that includes said lines (line 11, Algorithm \ref{alg:tool-workflow}).
% Like the previous request, we feed the patch and its summary and expect a list of code lines with their associated numbers as output.
% Next, we retrieve the function holding the requested code line from the project's repository (line 11, Algorithm \ref{alg:tool-workflow}). 
% After getting the supportive information, \toolName\ is ready to ask the LLM to provide the review comments.

\subsubsection{Related comment examples (\textbf{Example})}
As we consider the few-shot in our comment generation prompt, the default approach we use is to feed to the model a limited set of randomly selected examples of chunks with their associated review comments. 

The \textit{Example} approach improves on the default set of examples, by selecting relevant examples: examples are chosen based on their similarity to the current patch.
To do so, we first constructed a dataset of past chunks for each project source and their associated comment (tuples $(chunk, com)$). \Do{add the filtering thing} The examples are loaded in a QDrant dataset~\Do{add ref} and are retrieved using the cosine distance between chunks' embeddings. We retrieve 10 examples for each chunk in a patch, then report the top 10 examples out of all examples for the patch.

\subsection{Generating Code Reviews}
All the information retrieved in the previous steps is given as input to the LLM when asking for the code review.
This information is sequentially structured into a memory conversation buffer (see (4) in Table~\ref{tab:prompts}), which is responsible for providing the task context.
First, we set up the LLM to assume the persona of an expert code reviewer.
Second, we feed as LLM input the patch summary, providing context for the changes under analysis (line 4, Algorithm \ref{alg:tool-workflow}).
If functions and context lines are available based on previous steps, they are added to the buffer (lines 9 and 12, Algorithm \ref{alg:tool-workflow}).

Finally, \toolName\ asks the model to provide a code review: we instruct it to follow a \emph{few-shot} approach by providing examples of valid comments, aiming to guide the LLM to provide related and relevant content~\cite{nashid2023retrieval,brown2020language}. 
This way, we impose a standard pattern for the comments, consisting of the comment, associated line number, and file ($\{com;line;file\}$).
Once the LLM reports the comments (line 14, Algorithm~\ref{alg:tool-workflow}; prompt (5) shown in Table~\ref{tab:prompts}), \toolName\ makes one final request to filter out comments that do not address valid problems, by providing a list of undesired comment examples (\textit{undesired\_comments}).
The list of generated comments and its associated patch is given as input (line 15, Algorithm~\ref{alg:tool-workflow}; prompt (6) shown in Table~\ref{tab:prompts}).
Last, \toolName\ guides the LLM to report its results in JSON format (i.e., list of $\{com;line;file\}$).

% \subsection{Getting User's Feedback}
With the final list of comments generated (line 16, Algorithm~\ref{alg:tool-workflow}), \toolName\ stores all of them in a database server.
Next, based on the reported line numbers and file names associated with each comment, \toolName\ places the comments directly on the revision under analysis in the review interface.

\subsection{Technical Details}


GPT models are available online through an API, facilitating the process of prompting the models and escalating the number of requests.
% \toolName\ adopts the variant \texttt{GPT-4o} as its base LLM; we decided to consider this version, considering its advanced capabilities compared to previous models, based on our exploratory analysis.
\toolName\ leverage GPT4o as LLM with temperature 0.2; this allows the model to explore the most powerful LLM features available at the time of the study, but with a more focused and deterministic LLM configuration.
However, \toolName\ is open for extensions and could be adapted to work with different LLMs.


% Regarding storing the generated reviews, \toolName\ counts with the support of a database server...

\begin{comment}
        
General overview of information used to feed the LLM:
\begin{itemize}
    \item Getting the last diff of the code associated with a code review under progress through Phabricator;
    \item Splitting the diff at the file level (associated code line numbers);
    \item Getting additional code required by the LLM (function and context code)~\cite{ardito2020rust}.
\end{itemize}

\subsection{Running Code Reviews using LLMs}
General overview of information used to feed the LLM:
\begin{itemize}
    \item Ask the model to understand the codes under analysis~\cite{zheng2023take} and also for further information, if required;
    \item Few-shot approach adoption, based on previous findings that report LLMs achieve better results when using this approach~\cite{nashid2023retrieval,brown2020language};
    \item Chain-of-Thought regarding code summarization and additional required information~\cite{wei2022chain};
    \item Post-processing initial generated comments by filtering out irrelevant comments.
\end{itemize}

\subsection{Assisting Developers with Generated Comments}
\begin{itemize} 
    \item 
    \item Comments are individually presented and can be individually evaluated. Possible options: approve, reject, and ignore;
    \item When ignoring a comment, a developer is asked to provide additional feedback regarding their decision;
    \item In the end, all approved comments are posted at once.
\end{itemize}
\end{comment}



==> old/motivation_example.tex <==
To illustrate the problem addressed in this study, please consider the following scenarios when developers are assigned to perform different code reviews.
Initially, consider an initial bug reported on Bugzilla regarding Google Test (GTest) with ThreadSanitizer (TSAN) mode.\footnote{\href{https://bugzilla.mozilla.org/show_bug.cgi?id=1894419}{Bug Report - 1894419}}
After a developer is assigned to fix the bug, she applies the required changes and sends her contribution, leading to a new revision in Phabricator.\footnote{\href{https://phabricator.services.mozilla.com/D210979}{Fixing Revision for Bug - D210979}}
Before the assigned reviewer performs their review, a review bot is responsible for conducting some initial analysis.
In the current scenario, a linter, like ClangTidy, diagnoses and warns about a defect regarding a parameter that should be sent by reference and not by value.

Now, consider a new scenario when another developer addresses another bug reported on Bugzilla.\footnote{\href{https://bugzilla.mozilla.org/show_bug.cgi?id=1642476}{Bug Report - 1642476}}
Like the previous scenario, after the assigned developer is done with their contribution, a new revision is started on Phabricator.\footnote{\href{https://phabricator.services.mozilla.com/D77934}{Fixing Revision for Bug Report - D77934}}
This time, the review bot also reports some warnings focusing on typical programming errors.
Although the applicability of such bots is beneficial~\cite{wessel2020effects}, they share some limitations, as they typically report issues regarding style violations, interface misuse, or bugs detected via static analysis.
Knowing the complexity of the current revision, humans are required to take action in order to provide a review exploring the nuances of the code under analysis.

This way, developers assume the role of reviewers, adjusting their time to accomplish the new required tasks.
To provide good and valid reviews, developers should understand and reflect on the proposed changes in the overall system.
For such, they should check for possible associated parts of the system that the proposed changes could impact, like bugs or unhandled exceptions.
Such a task might be even more challenging for new teammates who are still learning about the system under analysis and the well-established practices and conventions. 
Besides the technical skills, reviewers must explore their social skills to provide reviews that are simple, concise, and direct~\cite{bogachenkova2022evaluating}. 

Such a scenario shows the complexity of performing code reviews and the eminent impact on developers' productivity.
Researchers have investigated different approaches to support developers when performing their reviews.
However, their assistive tools constantly require human intervention. 
Aiming to overcome these limitations and considering the potential of LLMs to perform NLP tasks, these assistive tools could be further extended, assisting reviewers when providing their reviews.

\begin{comment}

The code review process is commonly known by peers reviewing contributions of other peers.

Highlights of possible limitations faced by developers when providing code review:
\begin{itemize}
    \item Lack of knowledge;
    \item Limited time to perform the review, which includes checking for associated impacted code, consequently impacting the overall review quality;
    \item shallow feedback.
\end{itemize}
\end{comment}


==> tables/rq1_stats.tex <==
\begin{table}[t]
    \caption{RQ1: Fisher's statistical test's p-values when comparing Organization1 to Organization2 given a specific evaluation set and a metric.}
    \label{tab:rq1stat}
    \centering
    \begin{tabularx}{\linewidth}{l|X|X|X}
        \hline
        \backslashbox{\textbf{Metric}}{\textbf{Evaluation set}}& \textbf{Code} & \textbf{Example} & \textbf{Total}  \\
        \hline
         \textbf{Acceptance}&.363&.559&.296\\
         \textbf{Appreciation}&.696&.926&.975\\
        \hline
    \end{tabularx}
    
\end{table}

==> tables/rq2_type.tex <==

% \begin{table}[h]
%     \centering
%     \caption{RQ2 - Impact of the type of comments}
%     \label{tab:rq2type}
%     \begin{tabularx}{.47\textwidth}{rr|X|X|X|X}
%     \hline
%          \textbf{Comment}&& \multicolumn{2}{c|}{\textbf{Open-source}}& \multicolumn{2}{c}{\textbf{Closed-source}} \\
%         \textbf{category}& &RAG-Context&RAG-Examples&RAG-Context&RAG-Examples\\
%          \hline\hline
        %  Functional 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    & 11  & 8  \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Refactoring 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Discussion 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Tip 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        
% Accept & All & 0 & 0 & 13 & 25 \\
%  & Functional & NaN & NaN & 9 & 8 \\
%  & Refactoring & NaN & NaN & 4 & 17 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 0 \\
% \hline Useful & All & 0 & 0 & 20 & 20 \\
%  & Functional & NaN & NaN & 16 & 14 \\
%  & Refactoring & NaN & NaN & 4 & 4 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 2 \\
% \hline Ignore & All & 0 & 0 & 20 & 20 \\
%  & Functional & NaN & NaN & 16 & 12 \\
%  & Refactoring & NaN & NaN & 4 & 5 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 3 \\

% All labeled & Accept & 0 & 0 & 13 & 25 \\
%  & Useful & 0 & 0 & 20 & 20 \\
%  & Ignore & 0 & 0 & 20 & 20 \\
% \hline Functional & Accept & NaN & NaN & 9 & 8 \\
%  & Useful & NaN & NaN & 16 & 14 \\
%  & Ignore & NaN & NaN & 16 & 12 \\
% \hline Refactoring & Accept & NaN & NaN & 4 & 17 \\
%  & Useful & NaN & NaN & 4 & 4 \\
%  & Ignore & NaN & NaN & 4 & 5 \\
% \hline Documentation & Accept & NaN & NaN & 0 & 0 \\
%  & Useful & NaN & NaN & 0 & 0 \\
%  & Ignore & NaN & NaN & 0 & 0 \\
% \hline Discussion & Accept & NaN & NaN & 0 & 0 \\
%  & Useful & NaN & NaN & 0 & 2 \\
%  & Ignore & NaN & NaN & 0 & 3 \\
%         \hline
%     \end{tabularx}
% \end{table}



% \begin{table}[h]
%     \centering
%     \caption{RQ2 - Group of comments. "Sam" columns show counts from the samples where "Reb" represent the percentage of the original dataset size, rebalanced based on the true distribution of macro-evaluation. }
%     \label{tab:rq2type}
%     \begin{tabularx}{\linewidth}{p{.8cm}l|XX|XX|XX|XX}
%     \hline
%          && \multicolumn{4}{c|}{\textbf{Open-source}}& \multicolumn{4}{c}{\textbf{Closed-source}} \\
%         & &\multicolumn{2}{c|}{\textbf{Code}}&\multicolumn{2}{c|}{\textbf{Example}}&\multicolumn{2}{c|}
%         {\textbf{Code}}&\multicolumn{2}{c}{\textbf{Example}}\\
%         &&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb\\
%          \hline



% % \hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 13 & 8\% & 25 & 13\% \\
% %  & Valuable Tip & 0 & 0\% & 0 & 0\% & 20 & 42\% & 20 & 23\% \\
% %  & Rejected & 0 & 0\% & 0 & 0\% & 20 & 50\% & 20 & 63\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 53 & 100\% & 65 & 100\% \\
% % \hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & 9 & 6\% & 8 & 4\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 16 & 33\% & 14 & 16\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 16 & 40\% & 12 & 38\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 41 & 79\% & 34 & 59\% \\
% % \hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & 4 & 3\% & 17 & 9\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 4 & 8\% & 4 & 5\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 4 & 10\% & 5 & 16\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 12 & 21\% & 26 & 30\% \\
% % \hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
% % \hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 0 & 0\% & 2 & 2\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 3 & 9\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 5 & 12\% \\


% \hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 29 & 8\% & 50 & 13\% \\
%  & Valuable Tip & 0 & 0\% & 0 & 0\% & 35 & 42\% & 37 & 23\% \\
%  & Rejected & 0 & 0\% & 0 & 0\% & 37 & 50\% & 36 & 63\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 101 & 100\% & 123 & 100\% \\
% \hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & 14 & 4\% & 24 & 6\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 26 & 31\% & 27 & 17\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 29 & 39\% & 25 & 44\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 69 & 74\% & 76 & 67\% \\
% \hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & 13 & 4\% & 26 & 7\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 5 & 6\% & 7 & 4\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 7 & 9\% & 7 & 12\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 25 & 19\% & 40 & 24\% \\
% \hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 1 & 1\% & 0 & 0\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 1 & 1\% & 0 & 0\% \\
% \hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & 2 & 1\% & 0 & 0\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 3 & 4\% & 3 & 2\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 1 & 1\% & 4 & 7\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 6 & 5\% & 7 & 9\% \\
%          \hline
%     \end{tabularx}
% \end{table}



\begin{table*}[t]
    \centering
    \caption{RQ2 - Group of comments. "Sam" columns show counts from the samples where "Reb" represent the percentage of the original dataset size, rebalanced based on the true distribution of macro-evaluation. }
    \label{tab:rq2type}
    \begin{tabularx}{\textwidth}{ll|XXXXXX|XX||XXXX|XX}
    \hline
         && \multicolumn{8}{c||}{\textbf{Open-source}}& \multicolumn{6}{c}{\textbf{Closed-source}} \\
         & &\multicolumn{6}{c|}{\textbf{Approach}}&&&\multicolumn{4}{c}{\textbf{Approach}}
&&\\
        & &\multicolumn{2}{c}{\textbf{Code}}&\multicolumn{2}{c}{\textbf{Example}}&\multicolumn{2}{c|}{\textbf{Both}}&\multicolumn{2}{c|}{\textbf{Total}}&\multicolumn{2}{c}
        {\textbf{Code}}&\multicolumn{2}{c|}{\textbf{Example}}&\multicolumn{2}{c}{\textbf{Total}}\\
        &&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb\\
         \hline
\hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 29 & 8\% & 50 & 13\% & 79 & 11\% \\
 & Valuable Tip & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 35 & 42\% & 37 & 23\% & 72 & 32\% \\
 & Rejected & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 37 & 50\% & 36 & 63\% & 73 & 57\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 101 & 100\% & 123 & 100\% & 224 & 100\% \\
\hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 14 & 4\% & 24 & 6\% & 38 & 5\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 26 & 31\% & 27 & 17\% & 53 & 24\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 29 & 39\% & 25 & 44\% & 54 & 42\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 69 & 74\% & 76 & 67\% & 145 & 71\% \\
\hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 13 & 4\% & 26 & 7\% & 39 & 5\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 5 & 6\% & 7 & 4\% & 12 & 5\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 7 & 9\% & 7 & 12\% & 14 & 11\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 25 & 19\% & 40 & 24\% & 65 & 22\% \\
\hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 1 & 1\% & 0 & 0\% & 1 & 0\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 1 & 1\% & 0 & 0\% & 1 & 0\% \\
\hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 2 & 1\% & 0 & 0\% & 2 & 0\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 3 & 4\% & 3 & 2\% & 6 & 3\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 1 & 1\% & 4 & 7\% & 5 & 4\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 6 & 5\% & 7 & 9\% & 13 & 7\% \\

    \end{tabularx}
\end{table*}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/algorithms/tool.tex <==

\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}


\begin{algorithm}[t]
    \caption{\toolName\ Workflow. The (x) notation refers to the corresponding prompt in Table~\ref{tab:prompts}.}
    \label{alg:tool-workflow}
    {\fontsize{9pt}{9pt}\selectfont
    \SetAlgoLined
    \KwData{$patch$, $approach$}

    \KwResult{$code\_review$}
    
    % \textbf{Output:} $code\_review$

    \uIf{$patchNeedsReview(patch.status)$}{
            % \uIf{$countTokens(revision.patch)$ <= 3000}{
                
                $fpatch \leftarrow format(patch.sourcecode)$
                
                $sum \leftarrow askLLMforSummary(fpatch)$ (1)

                $mem \leftarrow createMemory([sum ])$ (4)

                \uIf{approach = Code}{
                $funcs \leftarrow askLLMNeedsFuncs(fpatch)$ (2)

                $lines \leftarrow askLLMNeedsLines(fpatch)$ (3)
                
                %$buffer.\text{append}(sum)$
                
                \uIf{$funcs.\text{size}$ $>$ 0}{
                    $context\_funcs \leftarrow getContext(funcs)$
                    
                    $mem.\text{addToMemory}(context\_funcs)$ (4)
                }

                \uIf{$lines.\text{size}$ $>$ 0}{
                    $context\_lines \leftarrow getContext(lines)$
                
                    $mem.\text{addToMemory}(context\_lines)$ (4)
                
                }
                
                $ex \leftarrow default\_set\_of\_few\_shot\_examples$
                
                }      

                \uElseIf{approach = Example}{
                $ex \leftarrow getSimilarExamples(fpatch)$
                }
                $first\_review \leftarrow askLLMReview(fpatch, mem,$ $ex)$ (5)
                
                $code\_review = askLLMFilterGeneration(fpatch,$
                $first\_review)$ (6)

                \Return $code\_review$
            % }
            % \Else{
            %     %\tcp{Patch is too large}
            %     \Throw{PatchSizeTooLarge}\;
            % }
        }
    % \Else{
    %     %\tcp{Patch does not require revision}
    %     \Throw{PatchHasNoStatusNeedsReview}{
    %     \# if the review is already done }
    %     }
    }
\end{algorithm}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/figures/RQ1_by_user.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{img/RQ1_acceptation_by_user.pdf}
    \caption{Acceptation rate [\%] by user.\Do{display will be fixed}}
    \label{fig:RQ1_by_user_acc}
    \includegraphics[width=.9\linewidth]{img/RQ1_appreciation_by_user.pdf}
    \caption{Appreciation rate [\%] by user.\Do{display will be fixed}}
    \label{fig:RQ1_by_user_app}
\end{figure}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/figures/RQ4_duration.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/rq4_duration.pdf}
    \caption{RQ3 - Evaluation duration. Outliers are hidden for visibility. }
    \label{fig:RQ4_duration}
\end{figure}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/1-introduction.tex <==
% \Do{some vocabulary choices for words that have multiple options: codebase (not code base), data point (not datapoint), chunk (not hunk, code snippet), patch (not pull request), exact match (not perfect match), generated comments (not suggestions), organization (not company), review environment (not tool), signaling (not signalling), behavior (not behaviour)}


Software code review is a core practice for modern software quality assurance~\cite{morales2015code,mcintosh2016empirical}, widely adopted in industrial and open-source projects ~\cite{sadowski2018modern,beller2014modern}.
While, initially, code review mostly was a synonym for code inspections on a submitted patch (structured as a set of chunks, i.e., successive lines of modified code)~\cite{bosu2017process,wang2015comparative},
the field gradually adopted a more dynamic approach to performing reviews commonly known as \emph{modern code reviews}~\cite{bacchelli2013expectations}, embracing social dimensions, like facilitating knowledge transfer between developers and strengthening synergy within teams~\cite{pangsakulyanont2014assessing}.

Despite such benefits, code reviews can also bring additional costs, due to the delay between a patch submission and its final approval for integration by the reviewers caused by back-and-forth between its author and reviewers~\cite{pascarella2018information}.
Additionally, providing valid and effective reviews requires non-trivial efforts from reviewers in terms of technical, social, and personal aspects~\cite{ebert2021exploratory}.
Reviewers need to understand and rationalize the overall impact of the changes under analysis while using effective communication~\cite{wurzel2023competencies,chouchen2021anti,paul2021security}.
Reviewers, even when qualified and focused on a patch, might miss issues due to fatigue~\cite{baum2019associating}, distraction, or pressure from other deadlines~\cite{shahin2017continuous}.


% To overcome these limitations, the research community has explored different approaches to automate the code review process.
% Hong et al. explored the potential of using review comments for similar code contributions in the past as candidate comments for current contributions under review~\cite{hong2022commentfinder}.
% State-of-the-art (SOTA) approaches for review comment generation tasks have focused on the use of fine-tuned LLMs such as T5 and CodeT5~\cite{li2022automating,tufano2022using}.
% Tufano et al. found that despite the promising results of ChatGPT, the  pretrained LLM used  off-the-shelf, it provides poorer performance for tasks associated with review generation than SOTA approaches~\cite{tufano2024code}. 
% \fixes{In some cases, Tufano et al. report that ChatGPT's output points to meaningful comments, though they miss or contradict the main points raised by the human reviewer in the ground truth comment set.}{Although Tufano et al.~\cite{tufano2024code} reports that ChatGPT's outputs often miss or contradict the main points raised by the human reviewer, Retrieval Augmented Generation could improve on the off-the-shelf model's performance~\cite{zhao2024retrieval}, which we explore in our approach.}

% \Do{I removed the all description on the previous work as it is similar to background (saving space). The comments we discussed are integrated in background.}
% To overcome these limitations, the research community has explored different approaches to automate the code review process.
% Hong et al. explored the potential of using review comments for similar code contributions in the past as candidate comments for current contributions under review.
% State-of-the-art (SOTA) approaches for review comment generation tasks have focused on the use of fine-tuned LLMs such as T5 and CodeT5.
% % Tufano et al.,~\cite{tufano2021towards} take a different route by investigating how Deep Learning models could be adopted for providing and addressing code review comments suggestion and code refinement.
% % Finally, considering the advance of Large Language Models (LLMs) and their potential to perform tasks involving natural language processing, researchers have investigated using them for different tasks related to the code review process.
% % Guo et al.~\cite{guo2024exploring} investigated the feasibility of refining code tasks using ChatGPT based on previous associated code reviews.
% Tufano et al. found that despite the promising results of ChatGPT, the  pretrained LLM used  off-the-shelf, it provides poorer performance for tasks associated with review generation than SOTA approaches. 
%  % In some cases, Tufano et al. report that ChatGPT's output points to meaningful comments, though they miss or contradict the main points raised by the human reviewer in the ground truth comment set~\cite{tufano2024code}.
% In some cases, Tufano et al. report that ChatGPT's output points to meaningful comments, though they miss or contradict the main points raised by the human reviewer in the ground truth comment set.
% % For instance, whie the human reviewer complains about a given change, further supported by the SOTA, ChatGPT considers such a change a valid one.
% % While uptake of LLM-based approaches for code review generation is increasing, thus far these have only been evaluated using textual metrics such as BLEU score and Exact Match~\cite{tufano2022using, li2022automating, hong2022commentfinder}.
% While uptake of LLM-based approaches for code review generation is increasing, thus far these have only been evaluated using textual metrics such as BLEU score and Exact Match. None of those studies have assessed the usefulness and adoption by human reviewers of generated review comments in a real development context, although the task requires synergy with human reviewers' processes.
To overcome these limitations, the research community has explored different approaches to generate review comments with LLM-based approaches such as T5, CodeT5 and ChatGPT\cite{tufano2022using, li2022automating, tufano2024code}. However, thus far these have only been evaluated using textual metrics such as BLEU score and Exact Match, which are imperfect as they do not capture the actual impact and synergy the approach can have on reviewers~\cite{tufano2022using}. Furthermore, it is unclear how reviewers receive LLM-generated comments in the long-term, i.e., apart from their relevance, to what extent do generated comments solicit follow-up comments by the patch author or lead to follow-up patch revisions?

To fill in this gap, we conducted the first large-scale user study in a live setup involving two organizations, Mozilla and Ubisoft. 
% We invited a set of reviewers from the two organizations to participate in the user study addressing the RQs mentioned in the introduction.
%The targeted companies are two big scale international software development companies. 
Our choice for both an open-source (Mozilla) and closed-source (Ubisoft) organization is deliberate, since open-source codebases risk being 
part of the pretraining data of LLMs like GPT4o, yielding an unfair advantage in empirical studies.
Hence, this study also aims at investigating whether open-source organizations actually benefit from this potential advantage compared to closed-source organizations.

Spanning over 6 weeks, our user study involved 59 reviewers, covered 587 patch reviews, and led to the evaluation of 1.6k generated comments. 
During this study, we monitored the reviewers' interactions with the generated comments, assessed the impact of these comments on the review flow, and finally conducted a survey of the participating reviewers to gain insight into their perspectives, filled by 37/59 participants. 

For this evaluation, we built \textit{\toolName}, an LLM-based review assistant that generates review comments and that is easy to integrate into modern review environments.
\toolName{} builds on GPT4o and uses both (i) Retrieval Augmented Generation (RAG)~\cite{zhao2024retrieval} to enclose relevant information and ground the model on the project under analysis, and (ii) LLM-as-a-Judge~\cite{zheng2023judging} to leverage LLMs' capacity to evaluate generated content and discard irrelevant review comments.
In particular, we exploit two different approaches for \toolName:

\textit{\toolName{} with extra code context (Code):} inspired by Zhou et al.'s approach for code generation~\cite{zhou2022docprompting}, the model can request a code retrieval tool to provide {function definitions} and additional {code lines} from the codebase under analysis.

\textit{\toolName{} with related comment examples (Example):} like Parvez et al.'s approach for code summarization~\cite{parvez2021retrieval}, for each patch, the model dynamically selects few-shot examples of review comments similar to its chunks, then provides them to the LLM.


% \begin{itemize}
%     \item \textit{\toolName{} with extra code context (Code):} inspired by Zhou et al.'s approach for code generation~\cite{zhou2022docprompting}, the model can request a code retrieval tool to provide further information from the codebase under analysis, e.g., {function definitions} and additional {code lines}.
%     \item \textit{\toolName{} with related comment examples (Example):} inspired by Parvez et al.'s approach for code summarization~\cite{parvez2021retrieval}, for each patch, we dynamically selected examples of review comments similar to its chunks and provide them to the model as few-shot examples.
% \end{itemize}


% We evaluated the two \toolName{} approaches through a large user study involving two companies, Mozilla, which has a open-source codebase, and Ubisoft, which has a closed-source one. 
% Spanning over 6 weeks, the study involved 57 reviewers, covered 550+ code reviews, and led to the evaluation of 1.6k comments generated by \toolName. 
% During this study, we monitored the reviewers' interactions with the generated comments, assessed the impact of these comments on the review flow, and finally conducted a survey of the participating reviewers to gain insight into their perspective.  
% , available as a Firefox and Chrome plugin for review tools.
% The tool uses GPT4o of-the-shelf with few-shot and chain-of-though architecture.
% For a given contribution under review (\textit{patch}), review suggestions are directly provided to reviewers in their usual review tool interface, 
%to be used in their day-to-day review tasks.

% The reviewer may \emph{accept} or \emph{ignore} comments individually; additional feedback might be provided for the ignored comments, considering the reasons for the non-acceptance. 
% \Do{maybe hid this because not true in all cases} In the end, the accepted comments are posted, informing that the content was generated with the support of \toolName. 

% To evaluate \toolName, we perform an empirical study assessing the acceptance of comments generated by our tool and the impact on the code review process. 
% We randomly selected developers from two companies, the first company having its data available in open-source and the second being fully closed-source.
% For that, we select a group of XXXXX developers to use \toolName\ for XXXXX days.
% We collect and compare a set of metrics covering the previously mentioned dimensions under analysis from before and after the adoption of \toolName. 


% subsection{Research Questions}
% Knowing that the code review process plays an essential role in software development, we assess different dimensions in software engineering that \toolName\ could impact.
% This way, to guide our evaluation, we focus on research questions exploring the acceptance of code review comments by developers and their impact on team productivity and engagement.
% Below, we discuss our research questions:
This paper addresses the following research questions:

% \begin{itemize}
%    \item \textbf{RQ1:} \emph{To what extent can we use LLMs to assist developers when providing code reviews?} In this RQ, we aim to assess the potential of generating code reviews using LLMs. Besides feeding the code under analysis, we investigate whether and how additional information can be used as input as well. - Second study
\textbf{RQ1: \suggRQone} 

    % This RQ evaluates the reviewers' adoption of comments generated by \toolName{}. 
    Based on the participants' feedback in both organizations, we found that 8.1\% and 7.2\% of comments are accepted by Mozilla and Ubisoft reviewers, respectively, with 23\% and 28.3\% other comments still appreciated as being helpful.
    % We also observe that 11-26\% of other comments are marked as valuable, as they provide tips that are helpful for reviewers or could even be used at earlier stages of development.
    % Considering both accepted and valuable changes, we report an appreciation ratio of 19.9-34\%.
    % Differences in source's origins could give an advantage to Mozilla, as the pre-trained LLMs could have had access to data and thus knowledge about their codebase.
    Despite the organizations differences in data availability, both the acceptance and appreciation ratios were consistent among them, indicating that the results may generalize across closed- and open-source development processes.
    Across both organizations, 23/37 participants reported they would continue using \toolName\ at least sometimes outside of the study context.
    
\textbf{RQ2: \suggRQtwo}

    % This RQ analyzes the type of issues pointed out by the generated review comments.
    We found that, for Mozilla and Ubisoft respectively,
    79.2\% and 84.9\% of generated comments are classified as functional issues, and 15.8\% and 14.5\% as refactoring-related comments.
    Furthermore, we found that refactoring-related comments have higher acceptance ratios than functional comments (18.2\% and 18.6\% compared to 4.8\% and 5.2\%).

\textbf{RQ3: \suggRQthree}

    % This RQ investigates the overhead introduced by \toolName\ on reviewers and their activity.
    % We measure the time spent analyzing the generated comments, evaluating them, and potentially editing them when accepted.
    % We also analyze the type of edits performed on the accepted review comments to identify opportunities for future improvement that can be applied to the format and content of generated comments.
    We find that, although reviews take longer due to the extra time needed to evaluate the generated comments, the time spent per generated comment is reasonable (43s as a median per patch). 
    This time is mostly spent on investigating the validity of the comment and on editing the comment when applicable, as 37/119 accepted comments were edited, with 25/37 cases being shortening the comment.
    
   
    %todo: check the dimensions evaluated by related studies.
    %todo: refactor RQ3
    %todo: Check ASE papers to structure the idea.
    
    %\lm{I think in one of our meetings, someone mentioned how the tool could impact developer interactions. In case we keep RQ4, we can even merge it within RQ3, as the scope is still about engagement, as Marco suggested today in our meeting (May 1).}
   % \item \textbf{RQ4:} \emph{How assertive are the comments generated by LLMs?} Knowing that code review comments might sometimes be subjective or inaccurate, leading to back-and-forth communication among developers, we also assess how \toolName impacts the communication among developers. For that, we compare the number of replies posted after a given comment. 
    %TODO: assessing engagement through the number of replies and also the time associated with them.

\textbf{RQ4: \suggRQfour} %\lm{Rephrase it. avoid the term productivity} regarding the delay in performing code reviews?} 
   
    This RQ assesses the extent to which accepted generated comments lead to changes in the codebase. 
    We found that accepted review comments lead to as many patch revisions (i.e., changes in a future version of the patch) as human comments (74\% vs 73\% at chunk level) in Ubisoft, indicating that the generated comments have the same impact as human comments.
    Also, generated comments lead to fewer follow-up comments among developers (23\% compared to 34\%).
    
    % , which is expected as the discussion comments are uncommon due to the prompt's design (less than 2\%).
    % changes the way reviewers and developers handle the code reviewer process.
    % For that, we compare the engagement before and after \toolName\ from two perspectives.
    % In the first one, we assess the dimension associated with the reviewer, exploring the contents of their reviews. 
    % For the second perspective, knowing that code review comments might sometimes be subjective or inaccurate, leading to back-and-forth communication among reviewers and developers, we explore the developer's side by assessing the replies/threads posted for a code review comment.
    

% Our results show that...

The main contributions of this study are:
\begin{itemize}
    % \item \toolName, an LLM-based assistive tool for supporting developers when performing code review;
    \item A large-scale mixed closed-/open-source user study, with 57 expert reviewers, assessing the usefulness of LLM-generated review comments and their impact on the review flow and outcome;
    \item A diverse set of 3.4k generated code review comments by GPT4o for the Mozilla organization, among which 426 were evaluated by reviewers~\cite{datamoz};% \Do{this is the Mozilla dataset only. Note here that Mozilla pre-generated the comments which leads to 3.4k generated ones and only 426 where evaluated.}
    \item An open source project implementing the comment review generation approach~\cite{bugbug}. 
\end{itemize}

% The rest of the paper is organized as follows.

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/1.5-related-work.tex <==
% This section discusses the related work to our proposed tool. 
% First, we present studies focusing on generic automation of the code review process. 
% Next, we will discuss the application of LLMs for related tasks.

\subsection{Automating the Code Review Process}
Previous studies have proposed a variety of approaches to automate different stages of the code review process.
For example, one category of studies focuses on recommending reviewers for a given patch~\cite{al2020workload,ouni2016search}.
Other studies investigate code change quality prediction, i.e., the best location in a submitted patch where review comments should be added~\cite{li2022automating,hellendoorn2021towards,shi2019automatic,hong2022should}.
Such approaches can assist the review process by either signaling that a chunk of code should be focused on~\cite{henley2018cfar}, or reordering files to show problematic parts of the patch first~\cite{olewicki2024empirical}.
% Hellendoorn et al.~\cite{hellendoorn2021towards} investigate which chunks of a given patch should be evaluated first, if any. 
% Li et al. explored the identification of parts (e.g., lines or chunks) of the code change that the reviewer should focus on~\cite{li2022automating}. 
% Their approach ``CodeReviewer" uses a Text-To-Text Transfer Transformer (T5).
% Shi et al. explore how the diff between two versions of a codebase can be used as context for a deep learning model to determine whether such a change might be accepted or rejected~\cite{shi2019automatic}. %Moved from line 9.
% Hong et al. proposed the ``RevSpot" approach to predict lines that should be commented on or revised~\cite{hong2022should}. 
% Evaluation of submitted code change's quality can 
However, they still rely on human effort to perform the review, which can be a time-consuming task~\cite{macleod2017code}.

% Previous studies have proposed a variety of approaches to automate different stages of the code review process.
% For example, one category of studies focuses on recommending the right reviewer for a given patch~\cite{al2020workload,ouni2016search}.
% Other studies investigate code change quality prediction, i.e., the best location in a submitted patch where review comments should be added, which can assist the review process by either signalling that a code snippet should be focused on~\cite{henley2018cfar}, or reordering files to show problematic parts of the patch first~\cite{olewicki2024empirical}.
% Hellendoorn et al.~\cite{hellendoorn2021towards} investigate which chunks of a given patch should be evaluated first, if any. 
% Li et al. explored the identification of parts (e.g., lines or chunks) of the code change that the reviewer should focus on~\cite{li2022automating}. 
% Their approach ``CodeReviewer" uses a Text-To-Text Transfer Transformer (T5).
% Shi et al. explore how the diff between two versions of a codebase can be used as context for a deep learning model to determine whether such a change might be accepted or rejected~\cite{shi2019automatic}. %Moved from line 9.
% Hong et al. proposed the ``RevSpot" approach to predict lines that should be commented on or revised~\cite{hong2022should}. 
% % Evaluation of submitted code change's quality can 
% However, all these approaches still rely on human effort to perform the review, which can be a time-consuming task~\cite{macleod2017code}.

\subsection{Review Comment Suggestion}

The field of review comment recommendation studies the generation of comments for a submitted patch.
Over the years, several such approaches have been proposed, which either represent code changes using tokenization~\cite{gupta2018intelligent, siow2020core}, word- and character-level embeddings~\cite{siow2020core}, or bag-of-words approaches~\cite{tufano2021towards, tufano2022using, li2022automating, hong2022commentfinder}. 
% Large Language Models (LLM) such as LSTM~\cite{gupta2018intelligent}, Bi-LSTM~\cite{siow2020core}, T5~\cite{tufano2021towards,tufano2022using} and CodeT5~\cite{li2022automating}, have been used to address the comment generation task. 
State-of-the-art (SOTA) approaches for review comment generation leverage custom LLMs such as T5 and CodeT5~\cite{li2022automating,tufano2022using}.
% Tufalo et al.'s approach was established as a state-of-the-art LLM approach in 2022~\cite{tufano2022using}, using T5.
% Then, Li et al.~\cite{li2022automating}'s proposal extended on Tufano et al.'s with CodeT5. 
% Regarding adopting LLMs to perform code reviews, researchers have been exploring different approaches and usages to achieve such a goal.
Tufano et al.~\cite{tufano2024code} compare these LLM-based SOTA approaches for code review generation to ChatGPT used in a zero-shot cognitive architecture, i.e., without any customization.
% By manually analyzing generated reviews, they propose a taxonomy of comment types, highlighting the topics that SOTA struggles and succeeds with. 
% The authors report that\fixes{ ChaptGPT as-is performs slightly better on coding tasks while struggling with different aspects when generating code reviews.}{, in some cases, ChatGPT's output points to meaningful comments, though they miss or contradict the main points raised by the human reviewer in the ground truth comment set~\cite{tufano2024code}.}
Although the authors report that ChatGPT's outputs often miss or contradict the main points raised by the human reviewer, the use of zero-shot prompting suggests that the use of additional context, e.g., using Retrieval Augmented Generation, could still improve on the off-the-shelf model's performance~\cite{zhao2024retrieval}, which we explore in this paper.



Hong et al.~\cite{hong2022commentfinder} propose \emph{CommentFinder}, a tool that retrieves past code review comments of similar patches and reports them as-is for the current patch under review.
% The authors transform patches into code token vectors based on the Bag-of-Words model.
% For a piece of code, the tool retrieves the closest code in the previous dataset, checking their similarity through the cosine metric.
They motivate their approach based on many other studies that found simpler approaches to be similar or even better than Deep Learning (DL) approaches in the context of software engineering (SE) tasks in terms of performance~\cite{fu2017easy,hellendoorn2017deep} and speed~\cite{majumder2018500}.
We believe that generative approaches could take advantage of \emph{CommentFinder}'s idea of selecting comments associated with the patch under review as few-shot examples in the prompt, which we considered in our study. 

Prior work~\cite{tufano2021towards,li2022automating,hong2022commentfinder} uses traditional NLP metrics, such as BLEU score (i.e., a metric of text translation quality) and Exact Match (i.e., the prediction matching exactly the expected output). 
% However, such metrics report low score on the task, the first being of around 5\% and the second around 3\%~\cite{li2022automating,tufano2022using}.
% Tufano et al. extend their evaluation with a manual validation of 100 comments that were not perfectly predicted, out of which 36 are semantically equivalent to the expected comment and 10 are an alternative solution~\cite{tufano2022using}. 
While Tufano et al. report BLEU scores around 5\% and Exact Match of 3\%, they suggest that these metrics are not perfect, and might thus under-evaluate the model's performance~\cite{tufano2022using}. Hence, the need for either investigating the creation of better metrics or conducting user studies and manual validations by experts: while previous work considered the former~\cite{huang2024empirical}. While Unzicker et al. conducted a user study to evaluate through a survey the impact of LLMs on mental workload and performance regarding the review comment generation task~\cite{unzicker2024all}, we evaluate its acceptance and usage of generated comments in day-to-day reviews.


% Moving on to automate the review process, machine learning algorithms have been explored to achieve this goal.


\subsection{Leveraging LLMs and Prompt Engineering}

% \bram{note from thesis: insist on chain-of-thoughs} \Do{}

Amidst the many LLMs currently available, GPT, a family of LLMs developed by OpenAI, currently stands out as one of the most popular LLMs. 
GPT has been used for a variety of applications, among which SE use cases like code generation, summarization, testing, and documentation \cite{zheng2023towards, ozkaya2023application}.

To guide LLMs like GPT in performing specific tasks accurately, users make requests to LLMs through textual prompts.
This process of defining, maintaining, and improving prompts is the subject of Prompt Engineering, a field that combines artificial intelligence and NLP tasks~\cite{beurer2023prompting}.
Various prompting patterns have been proposed to structure prompts more effectively.
For instance, while \emph{zero-shot} prompts rely exclusively on textual instructions given directly to an LLM~\cite{radford2019language}, \emph{few-shot} approaches provide more explicit context to the LLM by including concrete examples provided by the LLM user, to guide the LLM towards the expected behavior~\cite{nashid2023retrieval,brown2020language}. 
\emph{Chain-of-Thought} consists of providing a set of intermediate reasoning steps in the textual instructions, supporting the LLM to address tasks that require complex reasoning~\cite{wei2022chain}.

To improve the quality of a model's output, several techniques have been proposed. For instance, a user's prompt may specify constraints in terms of the style, structure, or type of answer expected from the model.
Among those, the prompt can suggest intrinsic characteristics like human pre-defined behavior patterns or persona that the LLM should inpersonate~\cite{white2023prompt}.
Also, \emph{Retrieval-Augmented Generation} can be used to
enhance the prompt with extra information relevant to the prompt retrieved from a corpus of user-provided documents, before the enriched prompt is sent to the LLM~\cite{zhao2024retrieval}. For instance, RAG has been used in SE for code generation~\cite{zhou2022docprompting} and code summarization~\cite{parvez2021retrieval}.
Finally, \textit{LLM-as-a-Judge} leverages the capacity of an LLM to auto-evaluate its generated content, which can be used to improve review comment generation through filtering or iterative generation~\cite{zheng2023judging}.
Our review comment generation approach integrates those different advances in LLM prompting.

% \Do{Hidden section here, need to check if the content is needed.}

% \subsection{Leveraging Code Review with LLMs}

% % Regarding adopting LLMs to perform code reviews, researchers have been exploring different approaches and usages to achieve such a goal.
% % Tufano et al.~\cite{tufano2024code} investigate the capabilities of SOTA tools for code review generation and how the generated contents compare with ChatGPT.
% % By manually analyzing generated reviews, they propose a taxonomy of types, highlighting the topics that SOTA struggles and succeeds with. 
% % Regarding the comparison with the ChatGPT, the authors report that the LLM performs slightly better on coding tasks while struggling with different aspects when generating code reviews.
% % Similar to our study... \lm{Compare with our results.}

% Yu et al.~\cite{yu2024security} investigate the potential of different LLMs to perform code reviews focusing on detecting security issues.
% For that, the authors select six versions from three different LLMs, adopting five prompts feeding different content.
% ChatGPT-4 presents the best performance, although facing some issues, highlighting conciseness problems, including unnecessary, irrelevant, and redundant reviews.
% In previous versions of our tool, we also observed such weaknesses; we tried to address them by adding an extra prompt advising the LLM to rethink the proposed comments and possibly remove them.
% % \lm{Compare with our results...}
% Similarly, Panichella~\cite{panichella2024vulnerabilities} discusses the occurrence of code vulnerabilities introduced by LLMs on recommended code snippets.
% % Although we do not use LLMs to generate code, regarding the generated reviews, we observe that... \lm{Bring some discussion about addressing vulnerabilities based on the manual evaluation.}

% Similar to our study, Watanabe et al.~\cite{watanabe2024use} investigate developers' perception of using ChatGPT to support code reviews in GitHub Pull Requests. 
% For that, the authors mined and categorized ChatGPT-generated comments based on their purposes. 
% Overall, developers use ChatGPT to perform tasks related to reference and outsourcing, including tasks not properly related to code review, like implementing changes and generating tests. 
% Regarding accepting ChatGPT comments, the authors report that 35 comments had negative answers, highlighting the need for filtering generated comments by reviewers.
% \toolName\ is focused on supporting reviewers when writing code reviews, allowing them to filter comments before sending comments to developers.

% Different of \toolName, Guo et al.~\cite{guo2024exploring} take a different route by exploring the potential of adopting LLMs to refine code under analysis based on code reviews.
% For that, they perform an empirical study comparing ChatGPT and \emph{CodeReviewer} (state-of-the-art tool) on different benchmarks. %of code review reports.
% The authors report that ChatGPT outperforms \emph{CodeReviewer} on code refinement tasks, highlighting its ability to perform better refinements considering high-quality reviews and refactoring-related tasks.  
% Frömmgen et al.~\cite{froemmgen2024resolving} explored the use of a T5 model for code refinement and report that 7.5\% of review comments are addressed by using the generated edits at Google, showing that such approach can be used for code refinement but also is being used in the review processes company-wide.
% Finally, Pornprasit and Tantithamthavorn \cite{pornprasit2024fine} investigate different prompts to leverage LLMs while also exploring fine-tuning these models, aiming to address code review comments.
% Overall, their results show that fine-tuning and few-shot techniques reported better performance.
% % \lm{The study reports that they achieved better results when not using a persona. Although we investigate a different problem that is still related, it could be interesting to investigate whether such a finding plays a role here.}
% Although the current version of \toolName\ does not support code refinement, the reported results reveal the feasibility of extending our tool while reaching a higher code review automation process.

% \lm{Discuss new related work}: \cite{yu2024fine}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/4-methodology.tex <==




Our goal is to evaluate the impact of integrating review comment generation into reviewers' workflow using a large-scale, mixed open-/closed-source user study. To do so, we developed a review assistant (\textit{\toolName}) that integrates easily into common review environments.
This section discusses the approaches used by \toolName\ and how the feedback of reviewers is gathered from the tool in the context of a user study.


\subsection{\toolName's LLM-based approach}
\label{sec:workflow}
% This section details the two LLM-based techniques for review comment generation's acceptance evaluated in our user study. 
\toolName{} relies on the following common LLM-based mechanisms: RAG (tool-LLM collaboration for code retrieval) and LLM-as-a-Judge through LLM-based evaluation. 
The approach leverage the Chain-of-Thought architecture, by splitting the overall review comment generation process %\fixes{}{and memory conversation ((4) in Table~\ref{tab:prompts})} 
into multiple prompts, some of which (i.e., prompts (5) and (6) in Table~\ref{tab:prompts}) also use Chain-of-Thought internally. Furthermore, a memory conversation is used to tie the prompts together ((4) in Table~\ref{tab:prompts}). %, with some  further decomposed into multiple steps. %\Do{just a note: I don't think we need to explain more than that about chain-of-thoughts. It is a quite common architecture and it's not the most recent technology we leverage, RAG and LLM-as-a-Judge are the approaches we need to explain more in this section}
%Then, we finally discuss the integration of the techniques into the review environments of the user study participants and how reviewers might interact with them.
In the following, we will describe the resulting workflow, summarized in Algorithm~\ref{alg:tool-workflow}.

\input{algorithms/tool}
\input{tables/prompts}

\subsubsection{Starting Point}
\toolName\ is automatically called when a reviewer opens a patch in their review environment.
Only patches labelled as \emph{Needs Review} are analyzed (line 1, Algorithm \ref{alg:tool-workflow}). 
% For a given patch, \toolName\ accesses the source code associated and starts to analyze it. 
Review comments are generated once per patch and kept in cache to maintain consistency if reviewers reload the page. 
Moreover, a reviewer will only be able to see any previously generated comments that have not yet been evaluated by another reviewer.

\toolName\ re-formats the patch to help the LLM understand the patch's content (line 2, Algorithm \ref{alg:tool-workflow}).
Knowing that a patch consists of one or more chunks (i.e., a sequence of changed lines), \toolName\ groups a patch's chunks per file while also adding the corresponding file line number to the beginning of each code line (instead of Git's default line number-range per chunk).
This allows the LLM to better associate the generated review comments with the target lines.
% Regarding informing the numbers of the code lines, we consider an efficient way to guide the tool in associating the provided review comments with the target lines.

% \begin{lstlisting}
% --- a/netwerk/streamconv/converters/mozTXTToHTMLConv.cpp
% +++ b/netwerk/streamconv/converters/mozTXTToHTMLConv.cpp
% @@ -1206,11 +1206,11 @@
%      } else {
%        uint32_t start = uint32_t(i);
%        i = aInString.FindChar('<', i);
%        if (i == kNotFound) i = lengthOfInString;

% -      nsString tempString;
% +      nsAutoStringN<256> tempString;
%        tempString.SetCapacity(uint32_t((uint32_t(i) - start) * growthRate));
%        UnescapeStr(uniBuffer, start, uint32_t(i) - start, tempString);
%        ScanTXT(tempString, whattodo, aOutString);
%      }
%    }
% \end{lstlisting}
Next, \toolName\ requests the LLM to summarize the formatted patch (line 3, Algorithm \ref{alg:tool-workflow}; prompt (1) in Table~\ref{tab:prompts}), using the LLM's ability to self-explain code~\cite{zheng2023take, wei2022chain,li2024approach}. 


\subsubsection{Extra context}~\label{approach_sec}
After generating the summary, \toolName{} seeks extra context to ground the model on the codebase under analysis and improve the quality of the generated comments. 
Building on the RAG mechanism, we consider two ways of providing extra context for comment generation, i.e., \textbf{\textit{Code}} and \textbf{\textit{Example}}. Although both approaches are complementary, in our user study on the impact of generated comments on the review process, we only considered one approach at a time.

\paragraph{Code context (\textbf{Code})}
Being aware that the patch under analysis might not contain sufficient details to perform a full analysis, we ask the LLM whether there are function calls referred by the patch that require the full function definition to understand its use (line 6, Algorithm \ref{alg:tool-workflow}).
For that, we feed the patch and its associated summary to the model, and request a list of the needed functions' names (prompt (2), Table~\ref{tab:prompts}).
Then, for each function name, a code retrieval tool accesses the respective project repository to retrieve the function's definition~\cite{ardito2020rust} (line 9, Algorithm \ref{alg:tool-workflow}) to provide to the model via the memory (line 10, Algorithm \ref{alg:tool-workflow}; conversation (4), Table~\ref{tab:prompts}).

Besides functions' definitions, other code context can also be needed for the model's review generation. In particular, the extracted code chunks only show up to 10 lines of context (i.e., unmodified lines above or below modified lines). This too might lead to missing context and hinder patch understanding.
Thus, we also ask the LLM whether it requires additional context for specific patch lines (line 7, Algorithm \ref{alg:tool-workflow}; prompt (3), Table~\ref{tab:prompts}), this time getting extended context around the requested lines by retrieving the functions that include said lines (line 12, Algorithm \ref{alg:tool-workflow}), then providing it to the memory (line 13, Algorithm \ref{alg:tool-workflow}; conversation (4), Table~\ref{tab:prompts}).

Finally, when using the \textit{Code} approach, the comment generation prompt (prompt (5), Table~\ref{tab:prompts}) will be provided with a fixed list of few-shot examples $ex$ randomly selected from past examples of chunks with their associated review comments (line 14, Algorithm \ref{alg:tool-workflow}). This default set is available in the replication package~\cite{bugbug}.

% By default, when not using the Code approach, the lists of function contexts are empty.
% Like the previous request, we feed the patch and its summary and expect a list of code lines with their associated numbers as output.
% Next, we retrieve the function holding the requested code line from the project's repository (line 11, Algorithm \ref{alg:tool-workflow}). 
% After getting the supportive information, \toolName\ is ready to ask the LLM to provide the review comments.

\paragraph{Related comment examples (\textbf{Example})} 
The \textit{Example} approach improves on the default set of examples provided by the \textit{Code} approach, by explicitly selecting relevant examples chosen based on their similarity to the current patch (line 16, Algorithm \ref{alg:tool-workflow}).
To do so, we first constructed a dataset for each studied project comprising past chunks and their associated comments (tuples of $(chunk, com)$), excluding tuples where the comment had more than 500 characters (to encourage concise comments only), or comments that included urls (which the model does not have access to). The examples are loaded in a vector database~\cite{qdrant} with GPT embeddings. Examples are retrieved from this database using the cosine distance between the embeddings of the current patch's chunks and the historical ones stored in the vector database. We retrieve 10 examples for each chunk in the current patch, then report the 10 examples with highest similarity out of all retrieved examples for the patch.

\subsubsection{Generating code reviews}
% All the information retrieved in the previous steps is given as input to the LLM when asking for the code review.
The information retrieved (i.e., summary and extra context) is sequentially structured into a memory conversation buffer ((4) in Table~\ref{tab:prompts}), which is responsible for providing the task context, including code context for the \textit{Code} approach and relevant examples for the \textit{Example} approach.
First, we set up the LLM to assume the persona of an expert reviewer.
Second, we feed the patch summary, providing context for the changes under analysis (line 4, Algorithm \ref{alg:tool-workflow}).
If functions and context lines are provided by the code retrieval tool based on previous steps, they are also added to the buffer (lines 10\&13, Algorithm \ref{alg:tool-workflow}).

Finally, \toolName\ asks the model to perform a code review (line 17, Algorithm \ref{alg:tool-workflow}; prompt (5) in Table~\ref{tab:prompts}): we instruct it to follow a \emph{few-shot} approach by providing examples of valid comments, either the default set or the retrieved set, aiming to guide the LLM to provide related and relevant content~\cite{nashid2023retrieval,brown2020language}. 
This way, we impose a standard pattern for the comments, consisting of the comment, associated line number, and file ($\{com;line;file\}$).

\subsubsection{Filtering generated comments}
Once the LLM has generated the comments, \toolName\ makes one final LLM-request in another conversation (i.e., without memory) to filter out comments that do not address valid problems.
Leveraging the concept of LLM-as-a-Judge~\cite{zheng2023judging}, \toolName{} prompts a filtering model providing the list of generated comments and the associated patch as input (line 18, Algorithm~\ref{alg:tool-workflow}; prompt (6) shown in Table~\ref{tab:prompts}). The model is also provided with a list of undesired comment examples (\textit{undesired\_comments}, which we constructed from preliminary feedback from a early users at Mozilla and iterations with the prompt) to guide the filtering process, which are available in our replication package~\cite{bugbug}.
Last, \toolName\ guides the LLM to report its results in JSON format (i.e., list of $\{com;line;file\}$).

% \subsection{Getting User's Feedback}
With the final list of comments generated (line 19, Algorithm~\ref{alg:tool-workflow}), \toolName\ stores them in a database server.
Based on the reported line numbers and file names associated with each comment, \toolName\ shows the generated comments directly on the patch under analysis in the review environment.

\subsubsection{Technical Details}


% GPT models are available online through an API, facilitating the process of prompting the models and scaling the number of requests.
% \toolName\ adopts the variant \texttt{GPT-4o} as its base LLM; we decided to consider this version, considering its advanced capabilities compared to previous models, based on our exploratory analysis.
After initial experiments, we decided on
%\toolName\ uses 
using GPT4o with a temperature of .2 to provide more accurate and deterministic results compared to higher temperatures, following Lin et al.~\cite{lin2024llm}.
For the embeddings used for the \textit{Example} approach, we used GPT text-embedding-3-large also with a .2 temperature. 
However, \toolName\ has been built for ease of extensibility and could be easily adapted to work with different LLMs and under different configurations.


\subsection{UI for \toolName's generated comments}
\label{sec:diffCompany}

% To evaluate the benefits and trade-offs associated with adopting \toolName, 
we integrated \toolName\ into participants' review environment, making it available to them when performing their day-to-day code review tasks.
Through the user study, reviewers can evaluate each generated comment, which is presented as a suggestion through an evaluation box shown in Figure~\ref{fig:eval}: ``add to comment" to \emph{accept} it or ``ignore" to \emph{reject} it.
In case of rejection, we additionally asked reviewers to provide a reason for ignoring comments, giving the options shown in Figure~\ref{fig:ignore}.
Before evaluating the comment, reviewers can also edit its content. 
Once evaluated, the evaluation box disappears, leaving no trace in the case of rejection and leaving a publicly published comment in the case of acceptance.
Each generated comment can only be evaluated once.

As the participating organizations use two different review environments (Mozilla uses Phabricator\footnote{Phabricator, accessed: 2024-10-15. \url{secure.phabricator.com/}}, while Ubisoft uses Swarm\footnote{Swarm, accessed: 2024-10-15. \url{www.perforce.com/products/helix-swarm}}), we also had to adapt \toolName\ to follow each organization's specific policies regarding reviews and generative-AI. This led to the following differences in design choices: 
% \begin{itemize}

\textit{Mozilla:} Accepted generated review comments had to be published as a separate reviewer named ``\textit{\toolName}". 
% by a service account, i.e., an account that clearly indicates that the comment was generated by AI, while also mentioning the name of the reviewer that accepted and edited the suggestion if applicable. 
The tool shows the generated comments' evaluation boxes directly when opening a review. 
In order to nudge the user study participants towards evaluating all review comments, the UI delays the publication of accepted generated comments to the patch author until all generated comments have been evaluated.

%\bram{Can each reviewer recover comments rejected earlier by another reviewer, or they are lost forever? In other words, are race conditions possible here?}
%\Do{I added something about this at the end of the first paragraph of "UI for RevMate. Regarding the race conditions, we did not test it out and I think that if two reviewers started at the same time the evaluation, we might have double evaluations, though it is highly unlikely (as it requires that they start in the same minute and as it would also have to be two participants of the study that happen to do the same review). anyway, the issue never occurred at Ubisoft has we only have single evaluations and at Mozilla I don't know if it overwrote the evaluations or skipped the update of the database if that happened, they also have only single evaluation.}

\textit{Ubisoft:} The reviewers had to publish the generated review comments that they accepted in their own name.
% This means that they can also modify the comment after accepting, which we track too. 
Furthermore, due to the review environment design and API, the generated comments could not be displayed immediately when opening the page. 
% Instead, reviewers needed to click on the proper line to have the suggestion displayed. 
To mark where generated comments were, we added a star symbol next to the lines on which reviewers needed to click for it to appear. 
To further help reviewers with finding the generated comments, for each file, we indicated next to the filename the comments' line numbers. 
% Reviewers were made aware of this design and were asked to click on those ``star" lines. 


For both organizations, a summary at the beginning of the patch's page tells users how many generated comments were generated and need to be evaluated.

\subsection{User study setup}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{img/eval_revmate.PNG}
    \caption{UI for generated comments' evaluation boxes}
    \label{fig:eval}
\end{figure}
\begin{figure}[t]   
    \centering 
    \includegraphics[width=.9\linewidth]{img/ignore_revmate.PNG}
    \caption{UI for choice of reasons for ignoring generated comments}
    \label{fig:ignore}
\end{figure}

We now discuss the setup of the user study that we designed to address the research questions listed in the introduction\footnote{Ethical approval: GREB Initial Ethics Clearance TRAQ\#6040278}.

\subsubsection{Participants and Target Projects} 
~\label{sec:companies}


Since our main goal is to evaluate the real-world potential of adopting LLMs as review assistant, we randomly contacted 50+ participants actively performing code reviews in ongoing projects in each organization. %\Do{I don't know how specific to be. at Ubisoft it was 58 people we contacted directly, at Mozilla, it was an open invitation sent through channels, but I don't know how many people were reached.}
% The projects are selected as they gather multiple hundreds of reviewers a months, with an average of \Do{Mozilla, do you have this number(s)?} XXXXX reviews a month for Company1 and \Do{Sarra can we share this?} 4k reviews a month for Company2.
The targeted projects all are mature projects that are continuously updated and written in different programming languages (e.g., C++, C\#).


As the contacted users joined on a voluntary base, we did not have control on the demographics. However, we can report that Mozilla had 28 participants with an average experience of 8.5~years inside the organization (from 1-13~years) and 13.4~years in their career (from 5-25~years), while Ubisoft had 31 participants, with average experience of 7.6~years inside the organization (from 1-25~years) and 10.9~years in their career (from 4-25~years). 
% development experience of 1-13 years (ave:8.5) inside the organization and 5-25 years (ave:13.4) in their career in general, while Organization2 had 31 participants, with experience in organization of 1-25 years (ave:7.6) and 4-25 ((ave:10.9) in their career. 

% In the case of Ubisoft, we invited 50 developers working on one of the main production in the company. The targeted project was chosen as it is an active production with multiple hundreds of employees participating in the development and review of the project.
% As a result, we can assess how \toolName\ works under patches written in multiple programming languages. 
% Meanwhile, aiming to reach diversity and cover multiple dimensions of the software development process, we consider different aspects when selecting the participants regarding gender, roles, seniority, and experience.
% \Do{COMMENT: Here we would maybe have a comment about not having restriction regarding gender? we don't select according to gender}\lm{Okay. I just brought up the discussion because reviewers always have a concern about it when it comes to evaluating tools.}
% Table Y summarizes the demographic information of our participants.
% Once the participants were selected, an initial training about how \toolName\ works was provided.
Before starting the study, a manual with instructions to install and run the tool in their specific review environment was sent to them.

\subsubsection{Running the Study}

Participants of the study within each organization are randomly split into two groups: one group gets the \textit{Code} approach and the other gets the \textit{Example} approach (see Section~\ref{approach_sec}). The differences between the two approaches are studied in RQ1.

For practical reasons, the study was conducted during 5~weeks at Mozilla and 6 at Ubisoft, covering respectively 165 and 422 code reviews assisted by \toolName.
The set of all generated reviews from Mozilla can be found in our online Appendix~\cite{datamoz}, whereas Ubisoft's data has to remain closed-source.


% \Do{COMMENT: only for Mozilla, Ubisoft will not be able to share the generated comments as they might include private information...}


% \end{itemize}
% Those policies lead to the following notable differences in design choices.

% For Company1, we showed the comments directly when opening a review. 
% Furthermore, we delayed the comment publication to the end of the evaluation of all suggestions, to enforce that reviewers needed to evaluate everything.

% In the case of Company2, the comments could not be displayed when opening the page due to the review tool design and API. 
% Reviewers needed to click on the proper line to have the suggestion displayed.
% To mark where suggestions were, we added a star symbol next to the lines.
% To further help them with finding the lines, for each file, we indicated next to the filename the line numbers where suggestions were made.
% Reviewers were made aware of this design and were asked to click on those ``star" lines. 


\subsection{Data Collection}

For each generated review comment, we gathered the following information: comment identifier, line number, filename, patch identifier, reviewer identifier, timestamp of evaluation, content of the generated comment, edited content (if applicable), evaluation (i.e., accept or ignore), reason (choice from list in Figure~\ref{fig:ignore}).
In the case of Ubisoft, we also have the timestamp on which the generated comment is opened, as users had to open them to read then evaluate them, which we used for RQ3.

After having access to the tool for a few weeks, we sent a survey to users to get their general feedback on the generative tool. The questions can be found in Table~\ref{tab:survey}.
Mozilla received responses from  15/28 participants, while Ubisoft received responses from 22/31 participants, for a total of 37 responses.

\input{tables/survey}

\subsection{Metrics and statistical tests}

%\Do{new section}

The accepted comments obviously represent high-quality generated comments, as they were adopted by reviewers. 
Hence, we analyze the acceptance ratio, $\frac{\#Accepted}{\#Evaluated}$, for both organizations.
However, among comments that were not accepted, some rejection motivations still indicate a positive impact for comments found to be useful as a tip for reviewers or during the development phase, which we will collectively refer to as ``Valuable Tips" ($\#ValuableTip$). We thus also report a second ratio, i.e., the appreciation ratio, $\frac{\#Accepted + \#ValuableTip}{\#Evaluated}$.


To compare proportions in our analysis, we use Fisher's statistical test, with $\alpha=.05$.
When the difference is statistically significant, we then use Cohen's d score ($CD$) to identify the effect~\cite{muller1989statistical}, with effect size small ($>$.2), medium ($>$.5), or large ($>$.8).



==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/5-results.tex <==


\section{RQ1: \suggRQone}

% \subsection{Motivation}

% \fixes{With this first question, we analyze how reviewers respond to \toolName's generated comments.}{}
% Although acceptance intuitively comes from publishing the suggested comment, we observed that even though some generated comments cannot be published as-is, reviewers also found value in LLM-generated comments, either as a tip for the reviewer or useful if it had been shown directly as a suggestion to the developer before submitting their work for code review.


\input{tables/rq1_eval}
\input{tables/rq1_res}
% \input{tables/rq1_stats}
% \input{figures/RQ1_by_user}
\subsection{Approach}

% During the user study, we monitored the participants' responses to the suggested review comments. 
In Table~\ref{tab:rq1eval}, we report numbers about the participants' evaluation of generated comments and, when applicable, their reasons for ignoring LLM-generated comments.
Even though participants were asked to evaluate all comments, we gave them the option to indicate cases where they felt unable to perform an evaluation (option ``Ignored - I'm not sure"). 
When considering all evaluated comments ($\#Evaluated$ in the ratios), we exclude those comments.

It should also be noted that due to differences in the review environment UI in the two organizations (see Section~\ref{sec:diffCompany}), reviewers from Ubisoft were not forced to evaluate the full set of generated comments per patch, but were encouraged to do so, contrary to Mozilla that enforced users to do full evaluations. 
This leads to comments that were seen but not evaluated in the case of Ubisoft, which we consider as ignored with no selected reason. We marked those as ``Ignore - Seen".
Acceptance and appreciation ratios are reported in Table~\ref{tab:rq1res}.
% \fixes{, while the results of statistical tests are reported in the following section.}{}
 % ($<$.05 is negligible, $<$.15 small, $<$.25 medium, else large)


% \Do{Before I also had a analysis for "by user" ratios but results are not really telling anything knew, compared to the results for the "by comment". So it's hidden for now.}

% As the results are impacted by how often users did comment evaluations, we also report ratios by reviewer in Figures~\ref{fig:RQ1_by_user_acc} and~\ref{fig:RQ1_by_user_app}. 
% We only report the results of reviewers that did more than 10 evaluations, so that the acceptance and appreciation are representative of an overall set of evaluation.
% We report statistical tests, using Mann-Whitney test and $\alpha=.05$, are reported in the following section.

\subsection{Results} \label{rq1res}

%\Do{suggested by bram: "Less than 10\% of generated comments were accepted (8.1\% for Mozilla, 7.2\% for Ubisoft), as can be seen in Table~\ref{tab:rq1res}." but I'm worried it's too negative so:}
\textbf{8.1\% and 7.2\% of generated comments were accepted, for Mozilla and Ubisoft respectively, as can be seen in Table~\ref{tab:rq1res}.}
For Ubisoft, the \textit{Example} approach reports a significantly better acceptance ratio (8.9\% vs 5.3\%) with a small effect size compared to the \textit{Code} approach (p-val=.011). For Mozilla, the \textit{Example} approach still reports a higher acceptance ratio (8.6\% vs 7.1\%), although the difference is not significant (p-val=.381). 
We suspect that the \textit{Example} approach has the advantage of showing comments more similar to what users are used to seeing and publishing themselves, as the few-shot examples shown by the \textit{Example} approach are taken from past similar published cases. 

%\Do{suggested by bram: "Less than 30\% generated comments, including than the accepted comments, are appreciated (23\% in Mozilla, 28.3\% in Ubisoft)." but I'm worried it's too negative so:}
\textbf{23\% and 28.3\% generated comments, comprising both accepted comments and valuable tips, are appreciated at Mozilla and Ubisoft respectively.}
Table~\ref{tab:rq1res} shows how, this time, the \textit{Code} approach reports a significantly higher appreciation (medium effect size) than the \textit{Example} approach, for both organizations (respectively, 29.9\% vs 19.9\% with p-val=.022 and 32.2\% vs 24.5\% with p-val=.002). 
This difference could indicate that the context related to the change provided by the \textit{Code} approach helps the model generate more informed and accurate comments. Yet, as the few-shot examples provided by this approach are quite limited compared to the \textit{Example} approach, and do not adapt to the precise style of comments required, the resulting comments do not seem to make it as publishable (accepted) review comments.%, as the approach does not see the style of comments as with .

% The significant difference in the case of Company2, which as fully closed-source code bases, could indicate that the additional context is especially valuable if the model was not pre-trained with data of the company.

\textbf{Overall, both organizations report similar results, despite their differences in codebase availability, development and review processes.}
% , as shown by our statistical analysis; p-values in Table~\ref{tab:rq1stat} all being higher than alpha=.05.
As indicated in Section~\ref{sec:companies}, Mozilla has the advantage that its codebase is open-source, with modern LLMs potentially having acquired knowledge about Mozilla's codebase through pre-training.
Yet, we do not observe any significant differences in results when comparing against each other both organizations, for any combination of ratios (i.e., acceptance and appreciation) and sets (i.e., Code, Example or Total) (p-value=.279 to .986).
% we observe that this advantage did not significantly impact the results.

% \textbf{}


\textbf{23/37 reviewers across both organizations reported that they would use a review assistive tool like \toolName\ at least sometimes outside of the study (question 5, Table~\ref{tab:survey}).} %\bram{can we list here some reasons why they say so before going to the bad news?} \Do{I tried rephrasing it by starting with positive (citations) then mentioning the negative but then we end with a negative note. Instead, I reformulated the first phrase to be more optimistic "mentioned that the relevancy of comments should be improved"}
% 10 participants reported they would rarely use such tool and none reported they would never use one.
To analyze this closer, two authors aggregated the participants' mentioned concerns from the open answers to question 4 of the survey, which asked users what they would change about the comments' content. 
% A participant mentioned that ``often looking at the suggestion help me think more about the code and reflect a bit more on what is done and why it is done." with 10 other making similar comment. Another mentioned that ``the tool can be super useful for less experienced reviewers and a good way for them to learn", with 3 users having similar feedback.
Overall, 20/37 participants explicitly mentioned that the relevancy of comments should be improved, as most of the suggested comments are ``\textit{accurate}", but ``\textit{superficial}" , ``\textit{obvious}", ``\textit{generic}", ``\textit{vague}", or sometimes even ``\textit{wrong}", as also confirmed by the numbers for ``Ignore - Trivial comment'' and ``Ignore - Incorrect comment'' in Table~\ref{tab:rq1eval}. 
Yet, one participant mentioned that ``\textit{the tool can be super useful for less experienced reviewers and a good way for them to learn}", confirmed by 2 other users.
Also, 6/37 mentioned being optimistic on the future of LLM-based approaches for review assistance tasks, and 11/37 mentioned that, at least, the tool was able to guide their review (i.e., providing a tip for reviewers).

%\Do{Those are insights from the survey, not through multiple choice but open question, so its not the same 20 person. I just report how many people mentioned what, not everyone actually responded to the open questions or addressed there choice}

\noindent\doublebox{%
    \parbox{.95\linewidth}{%
        \textbf{RQ1: Generated review comments achieve promising acceptance (8.1\% and 7.2\%) and appreciation ratios (23\% and 28.3\%). 23/37 reviewers that answered our survey reported that they would continue using \toolName~at least sometimes. %\bram{do we have any threshold to compare these numbers to? for instance, the performance results of the studies mentioned in related work section?}\Do{not comparable to other studies: different approach, different total ensemble (total out of comments generated VS out of diff that requires comment), diff metrics (acceptance and appreciation VS BLEU et EM). Due to that we could almost argue that we look at the precision (out of the ones we commented, how much were well commented) where they look at the recall (out of the ones they needed to comment, how much were well commented), but it's not even exactly the case. However, I added in background some numbers, so that people could get to their own conclusion that acceptance and appreciation are higher than the 5\% BLEU score of SOTA.}
        }
    }%
}

% \input{tables/rq2_type}
\input{tables/rq2_type_auto}
\section{RQ2: \suggRQtwo}

% \subsection{Motivation}

% \fixes{Apart from evaluating the overall generated comments, we wanted to see if specific comment categories are more commonly accepted, appreciated, or rejected.}{} 



\subsection{Approach}

% To label our dataset, we gathered comments into clusters with 
% \textit{KMeans}\footnote{Sklearn's KMeans, accessed:2024-10-15. \url{scikit-learn.org/1.5/modules/generated/sklearn.cluster.KMeans.html}}, then used GPT's text-embedding-3-large embedding to tag each cluster with a descriptive label~\cite{labelcluster}. 
To automatically categorize the generated comments, we clustered them according to their embeddings, then used an LLM to synthesize a category label for each cluster based on the comments that it contains\cite{labelcluster}. 
The categories we considered are the general categories presented by Turzo et al.~\cite{turzo2024makes}: functional, refactoring, documentation, and discussion.
% We validated the labels by comparing the generated cluster labels with a set of comments manually labelled as our ground truth:





% \textit{For the automated labelling of all comments:} 
% The automated labelling approach is based on clustering of comments according to their embeddings, then using an LLM to synthesize a label for each cluster based on the comments that it contains\cite{labelcluster}. 
First, comments are gathered into clusters using Kmeans\cite{kmean} on the embedded comment (using GPT's text-embedding-3-large).
Then, we ask the LLM to label each cluster of comments with a descriptive label, by providing it with a list of label examples of the form ``\textit{\{general\_category\} - \{specific\_category\}: \{description\}}'', corresponding to the table of categories presented by Turzo et al.~\cite{turzo2024makes}.
Given those examples, we observed that often, multiple clusters were labelled with the same label, which led us to eventually merge the 363/400 concerned clusters into the final 37 clusters shown in Table~\ref{tab:cluster}.
Also, not all generated labels existed in the original list of examples we provided, which we indicate by a star ``*" in Table~\ref{tab:cluster}.
We ran the LLM-base labelling 5 times and report for each comment the label that got the majority vote.

In order to determine the optimal number of clusters, we compared, for the number of clusters ranging from 2 to 400, the \textit{general\_category} of each cluster with that of a manually labelled ground truth, which we discuss below. We found that the percentage of matches with the ground truth converged between 300-400 clusters, leading to 76.3\% of matches (171/244) for 400 clusters, with only 37 distinct labels being generated even with that amount of clusters. 
To evaluate the agreement between the model and the ground truth (human labelling), we used Cohen's kappa score, a metric between -1 and +1 where +1 indicates total agreement and -1 total disagreement~\cite{cohen1960coefficient}. 
We obtained a kappa score of .45, which is considered as moderate but acceptable agreement.

To obtain the manually labelled ground truth, used to determine the optimal number of clusters, we sampled from each of the macro-evaluation categories of RQ1 (i.e., accepted, valuable tip, and rejected) 83 generated comments (70\% of \#accepted, the ones available at the time of the analysis), in order to have a balanced set of each type, for a total of 249 comments.
Then, two authors manually labelled each sample with a comment category using Turzo et al.'s main categories~\cite{turzo2024makes}.
We did not consider their ``false positive'' category, as we did not evaluate the validity of the comment, only its category. 
In the end, in 93\% of the cases (230/249) the authors agreed on the selection of one out of the four possible categories.
The kappa score between both authors' labelling of .83 is considered as almost perfect agreement.
For any conflicts, the two authors performing the labelling discussed and eventually agreed on the category using the \textit{negotiating agreement} technique~\cite{campbell2013coding}, but 5 comments were left unlabelled because of ambiguity in the comments themselves.
The latter were discarded, leaving us with 244 labelled comments.




% as two main parameters: the amount of clusters and the prompt. Approach is 

% We also indicated for each comments if it was "not-actionable", i.e. if the comment was to vague and did not suggest any change. \Do{show an example here}

% We report the number of comments of different groups and "not-actionable" attribution counts in Table~\ref{tab:rq2type}. 
% % It should be noted that the "Documentation" group was never encountered in the labeling, so we did not report it in the Table.

% To compute the acceptance and appreciation ratio per group of comment, we need to know the distribution of each group of comment accross all the generatiod comments.
% As we sampled balanced groups from the macro-evaluation types, we rebalanced each count based on the true size of of each types sub-set ($rebalanced\_count = \frac{true\_total}{sample\_size} count$).
% Then, we report the acceptance and appreciation ratios in Table~\ref{tab:rq1res}, based on those rebalanced counts, and we report statistical test, Fisher's test \Do{TODO} with $\alpha=.05$ in the following section.



For the selected number of clusters (400) and resulting cluster labels, we now split comments into groups according to the generated labels' \textit{general\_category}, shown in Table~\ref{tab:categoryres}, as well as their acceptance and appreciation ratios. 
% Although we discarded the \textit{specific\_categories} in our analysis, we used them as a sanity check to ensure that the LLM was not assigning the general categories randomly, by checking that the general categories were matched with relevant specific categories. \Do{please check if this phrase is clear. It was not a systematic analysis, just for us to check the connections made sense and the model was not fully hallucinating}\bram{why not just adding one paragraph in the results about the most common sub-categories? then we don't need to say that we discarded that data (since that sentence would cause reviewers to ask to either do something with it, or remove from the table)}\Do{todo}
% We perform the statistical test the same way as for RQ1.
% As we sampled balanced groups from the macro-evaluation types, we rebalanced each count based on the true size of of each types sub-set ($rebalanced\_count = \frac{true\_total}{sample\_size} count$).
% Then, we report the acceptance and appreciation ratios in Table~\ref{tab:rq1res}, based on those rebalanced counts, and we report statistical test, Fisher's test \Do{TODO} with $\alpha=.05$ in the following section.

\subsection{Results}

\textbf{Table~\ref{tab:categoryres} shows that Functional and Refactoring comments are the most commonly generated comments, with respectively 79.2\% and 15.8\% for Mozilla and 84.8\% and 14.5\% for Ubisoft.} 
Notably, Table~\ref{tab:cluster} shows that the most popular sub-categories of Functional comments are ``Validation'', ``Logical", ``Resource" and ``Interface", and ``Organization of the code" and ``Solution approach" in the case of Refactoring comments. Those subcategories were proposed through the few-shot examples provided to the LLM, from Turzo et al.~\cite{turzo2024makes}.
The Documentation and Discussion labels are the rarest, with a total of 21/418 comments for Mozilla and 8/1,185 for Ubisoft.
This is expected, as the prompt ``\textit{AskLLMReview}'' (see prompt (5) in Table~\ref{tab:prompts}) suggests that such comments are not desirable, which is also why we did not report their acceptance and appreciation ratios in Table~\ref{tab:categoryres}.


\textbf{Refactoring comments are accepted more than functional comments (18.2\% vs 4.8\% for Mozilla and 18.6\% vs 5.2\% for Ubisoft).}
This difference is statistically significant with large effect size, with respectively p-values .0 and .002. 

\textbf{In Mozilla, appreciation for refactoring comments is significantly higher than for functional comments (36.4\% vs 19\%, p-val=.002, large effect size).}
In the case of Ubisoft, the difference is not significant (p-val=.877), although in practice Functional comments are more appreciated (29\% vs 25\%).

\noindent\doublebox{%
    \parbox{.95\linewidth}{%
        \textbf{RQ2: Refactoring comments report a significantly higher acceptance ratio than Functional comments in most cases (18.2 vs 4.8\% for Mozilla and 18.6 vs 5.2\% for Ubisoft). Discussion and Documentation comments are rare (29/1,603 comments), which is expected based on our prompt design.
        }
    }%
}

\section{RQ3: \suggRQthree}

% \subsection{Motivation}

% \fixes{RQ3 aims to evaluate how the reviewers' interactions with the generated comments impacted their review process.}{}

\subsection{Approach}

In question 3 of the survey (Table~\ref{tab:survey}), we asked participants whether interacting with the generated comments impacted the duration of their reviews. 
In the case of Ubisoft, we also captured the time it took to evaluate the generated comments in order to empirically estimate that time.
This was possible due to the difference in design (see Section~\ref{sec:diffCompany}): for each generated comment, we marked the timestamp of when a given comment was first opened (not applicable to Mozilla) and of the timestamp when the reviewer submitted their evaluation of this comment. The difference between those timestamps provides an upper bound on the actual time it took a reviewer to evaluate a generated comment, as this period is longer than the actual time taken for evaluation due to switching to other comments or distractions.
% We exclude duration over 10min as they probably indicate that the reviewer did was interrupted, which filtered out 15 comments (2.5\%). 
In Figure~\ref{fig:RQ4_duration}'s boxplots, we report the distribution of the duration of evaluation per comment and per patch review (i.e., total duration for all its generated comments' evaluations).

\input{figures/RQ4_duration}

We also evaluate how reviewers edit the accepted review comments. In Table~\ref{tab:edits}, we report four different types of edits on accepted comments:
\begin{itemize}
    \item As-is: with no modification (i.e., exact match between generated and published comment);
    \item Shorten: the published comment is shorter than the generated one;
    \item Extended: the generated comment is included as-is in the published one, but more text was added around it;
    \item Other modification: any modification not included above.
    % \item Moved: The comment's line number differs from the suggestion line number (independently of any other modification).
\end{itemize} %that are 

\subsection{Results}
\input{tables/rq5_edits}

\textbf{The median time spent at Ubisoft on the evaluation of individual comments is 27.6s for accepted comments and 16s for others, as shown in Figure~\ref{fig:RQ4_duration}.} 
By 24/37 users in the survey, the additional effort of evaluating comments was reported as, to some extent, slowing down the review process. 
Our quantitative analysis of the comment timestamps showed that this slowdown is relatively limited, falling within a 95\% confidence interval of [1s,116s] (median of 27.6s) for accepted comments, and [1s,76s] (median of 16s) for others.
% We found that the median time spent on each suggestion evaluation is 27.6s for accepted comments and 16s for others.
Although time spent on ignored comments might be considered ``wasted time'' by reviewers, in some cases the comments might still inspire the reviewer to comment on the code about problems they would have missed otherwise, or at least force an extra verification of the code. We did not find any significant difference in the median time spent evaluating appreciated comments vs fully rejected comments, hence did not include the former in Fig.~\ref{fig:RQ4_duration}.%\bram{what about the duration for the appreciated comments vs. fully rejected comments?}\Do{ for "valuable comments" the time was not different from fully rejected, so I did not report the difference}

\textbf{By patch, the median total time spent on generated comments is 42.9sec (95\% confidence interval [5s,5min12s]).}
This effort is considered by many users as acceptable. For instance, one of the reviewers commented: \textit{``Often looking at the suggestion helps me think more about the code and reflect a bit more on what is done and why it is done. So overall, I think it is a bit slower to do reviews, but my reviews are actually better now that I use the tool"}.
Similar comments were made by 11/37 users.
The extra time spent on the generated comments also comes from either verifying the validity of the comment or, specifically for the accepted ones, modifying the comments.
%\bram{what is the normal duration of code reviews? is 5min12s big compared to the typical duration?}
%\Do{no source have really address this, other than our hot-spot paper reporting 11min for reviewers of 5 files. But here we did not compare regarding the size of review so I don't want to exploit this. To me the citation of the participant saying it was reasonable is already a good argument. + the time is a vague estimation, with potential disturbance when they did the review, so this should be mostly informative that they spend a reasonable time on generated content}

\textbf{27/34 accepted comments were published as-is for Mozilla, 55/85 for Ubisoft, as shown in Table~\ref{tab:edits}}
The most common type of edit to generated comments is to shorten the comment (6/34 for Mozilla, 19/85 for Ubisoft), which suggests that generated comments can often be too wordy, which was confirmed in the survey by three participants. %, hence the need for reviewers to change the comment. 
In future work, we want to iterate on the prompt to make generated comments more succinct. 


\noindent\doublebox{%
    \parbox{.95\linewidth}{%
        \textbf{RQ3: 24/37 surveyed reviewers report that review duration is increased by our tool. We quantitatively measured that the median time dedicated to the inspection of generated comments at the review level is 43s in Ubisoft, which users find reasonable. In both organizations, most comments, when accepted, are mostly published as-is (82/119) or shortened (25/119).
        }
    }%
}
% \section{RQ5: \suggRQfive}

% \Do{merged into workflow}
% \subsection{Motivation}
% \subsection{Approach}
% \subsection{Results}




\section{RQ4: \suggRQfour}

% \subsection{Motivation}

 % \fixes{This question analyzes how the accepted generated comments for a given patch impact the patch's review process regarding potential threads of review comments (i.e., where reviewers or authors respond to the published comment) or follow-up revisions, compared to other comments written by reviewers who did not use \toolName.}{}

\subsection{Approach}

To evaluate the impact of accepted comments on the further processing of the patch, we captured, for each line commented on via an accepted generated comment, whether that comment led to threads of review comments and/or follow-up revisions. 

A potential impact of the comment would be any follow-up review comments, i.e., threads of comments, made by the author of the patch or other reviewers in response to the posted comment to (1) better understand the needed change, (2) argue about the need for adjusted revisions suggested or (3) acknowledge the actions taken for the requested change.
% Those discussions can lead to potential improvement on the same patch or even motivate the need for future pull requests.
It should be noted that the follow-up revisions might not be directly related to the accepted comments, but at least this characteristic provides a reasonable approximation of the potential impact the comment may have had on the evaluation of the commented patch, in both generated comments and human comments from patch reviews outside of the user study. 

For the analysis of the impact of generated comments on later patch revisions and/or review discussions, we selected comments based on the following constraints.
First, we only consider accepted comments.
Then, we restricted the selection to patches with ``finished'' review status, since some reviews were still ongoing at the time of the study, thus the comment might not yet have been dealt with.
Finally, we considered only results from Ubisoft, which represent 69 comments satisfying the selection criteria, as Mozilla had only 25 cases after filtering, which would not have led to significant comparison. 

As a baseline for our analysis on generated comments, we also collected a dataset of ``Human" comments, by other reviewers not part of the user study, sampled randomly from patches under review in Ubisoft but that were not included in the actual user study, yielding a total of 1,211 comments.
% The count of each characteristics are reported in Table~\ref{tab:rq4res}. 
% We also report Organization1's impact counts, but we do not compare them with human comments as the generated set has only 25 cases. \Do{maybe we do not even show the results of Mozilla?} \bram{would be better, although it would not be bad to include a comparison for Mozilla as well, even with 25 case} \Do{we don't have the human examples from Mozilla}


% \textit{Revised line}: The line was modified in a follow-up revision.

% \textit{Revised chunk}: The line was modified or part of context in a follow-up patch revision.

% \textit{Thread}: A comment responds to the generated comment. 

% Each comment can have have the following characteristics:
We report in Table~\ref{tab:rq4res} three different types of impact that accepted comments can exhibit:

\begin{itemize}
    \item \textit{Revised line}: The comment's line was modified in a follow-up patch revision.

\item \textit{Revised chunk}: The comment's line was modified or was part of the context in a follow-up patch revision.

\item \textit{Thread}: There was a comment in response to it. 
\end{itemize}
% We report in Table~\ref{tab:rq4res} the number of comments having each characteristics and the percentage of comments concerned in comparison to the total set ($\%characteric =\frac{\#characteric}{\#total}$). \Do{move the ratio explanation to table?}


\subsection{Results}

\textbf{In Ubisoft, generated comments lead to as many revisions on the line (62.3\% and 64.3\%) and chunk level (73.9\% and 73.2\%) as human comments do.} 
No significant difference is found in revision ratios on either levels (p-val=.413 and p-val=.515, respectively). 
% Organization1 has 14/25 accepted comments that led to revisions.

\textbf{For Ubisoft, significantly less comment threads were started on generated comments (23.2\%) compared to human comments (33.9\%).}
The difference is statistically significant (p-val=.041) with medium effect size.
This is expected, as the generated comments are not meant to start discussions, whereas human comments can often, for instance, be phrased as genuine questions requesting a response.  %\bram{The patch author does not know that the comment is generated, so this sentence feels a bit odd, i.e., even if the comment is not a discussion thing but a technical observation, people could still have questions on how to do things in the best possible way?} \Do{yes, that's why generated comments can still start discussions, but human comments can purposefully start discussions (questions, discussion, etc.) where generated comments don't aim at that}
This expands on our findings from RQ2 that most comments are not of the Discussions category.
However, from manual inspection of the concerned comments, in practice the threads tend to discuss the generated comment and/or to acknowledge the change (i.e., writing ``Done'') or reject it.

\input{tables/rq4_impact}

\noindent\doublebox{%
    \parbox{.95\linewidth}{%
        \textbf{RQ4: Generated comments experienced as many revisions as human comments (73.9 vs 73.2\% at chunk-level), but less follow-up comments (23.2 vs 33.9\%). 
        }
    }%
}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/6-discussion.tex <==
% \subsection{Is review comment generation ready for prime-time?}

Evaluating review comment generation is a challenging task, especially as it is essential to capture the impact of assisting reviewers in their work.
Where prior work has addressed the question of review comment generation by textually comparing the generated outputs with a ground truth of past chunks commented on by humans, such metrics do not evaluate the impact the generation has on the reviewers' workflow.
In this paper, we instead carried out a user study to gather feedback from reviewers in two software development organizations. 

The first metric we report is acceptance, i.e., the ratio at which reviewers actually accepted comments for publication. 
We observed that reviewers, even if they ignore the comments, often still report them as having value (14.6\% and 20.5\%).

First, reviewers reported that 5.4\% and 12.8\% comments, respectively, could actually be more valuable for developers before they submit their patch. Those generated comments are thus shown too late in the development process.
One participant reported in the survey ``\textit{It detects perfectly possible flaws in the code, but most of the suggestions are more in the development realm than the review}", with 4 participants making similar comments. That reason for ignoring LLM-generated comments was used by 28/57 reviewers. 

Second, although some comments are not actionable as-is or not mentioning specific problems, they often (9.2\% and 7.7\%) raise interesting questions ``\textit{that force to look around, and it is what is found by looking around that is the most useful}", as mentioned by one participant. Another even suggests, ``\textit{there's more value in highlighting potential issues with a more concise explanation and let the reviewer write the comment}", and similar comments were provided by 10 other participants. The ``review tip" reason was used by 25/57 participants.

%Both types of valuable additions indicate that there is a relevant appreciation ratio for the generated comments (23\% and 28.3\%), though they are not always proper actionable comments. 
The high ratio of appreciation (23\% and 28.3\%) compared to comment acceptance highlights that the comment generation approach actually addresses multiple tasks: suggesting actionable comments, developer tips and review tips.
Future work should explore the possibility to split the overall review comment generation task by predicting the type of generated comments or specializing towards the generation of specific comment types. Developer tips should be shown ahead of the review process (perhaps giving developers access to tools like \toolName\ before patch submission), and review tips should be shown to reviewers differently than actionable comments, as they act as a warning for reviewers to focus on some specific code snippet.
The same observation can be done regarding categories of comments: future work could explore the categories of review comments, considering generation of each category as a separate task, and focus the generation on specific categories, depending on reviewers' preferences.

% \Do{I hid two paragraphs here (about first customization, which I simplified in the last sentence of the paragraph here above and second about improving the perf, because obvious improvement needed, we don't want to finish on the negative note}
% Furthermore, customizing the tool to reviewers’ needs, experience and preferences would improve the users' experience with review comment generation tools. A participant even suggested that the customization could depend on the patch author's experience, mentioning ``\textit{I would not add a trivial comment when reviewing the code of a tech lead, whereas I would add the trivial comment when reviewing the code of a junior developer}". \Do{Sarra mentioned maybe not mentioning this in paper to not be snatched}

% Finally, improvement on the LLM-based approaches used in order to generate more specific comments, or to filter out wrong and trivial comments would be necessary, as this is the biggest concern reported by participants: one reviewer mentioned ``\textit{A lot of suggestions I ended up dismissing, so I'd want to be able to filter out some of the noise and focus on the ones that were useful or caught genuine issues}". Similar comments were reported by 19 participants. \bram{this sounds quite negatively compared to that earlier RQ's findings} \Do{maybe hid both last paragraphs}






% \subsection{Habituation to \toolName}

% Over time, reviewers might get used to \toolName, possibly influencing their acceptance or rejection independently of the comments' quality. 
% However, as different patches are associated with supporting code, when applicable, we expect the comments to address different aspects, which reviewers might further check. 
% In the same way, reviewers might accept or reject comments based on their personal judgment and/or style of reviews. 
% For example, prioritizing comments addressing issues/bugs in the code under analysis, instead of also considering comments on documentation and code organization.
% When evaluating productivity, different factors, like deadlines, policies, and tool changes, might affect our results, which we cannot control during our investigation. 


% \subsection{Off-the-shelf vs Fine-tuned LLMs}

% LLMs are known to be expensive from a computational point of view, regarding both training and generation.
% The approach we consider uses an off-the-shelf model with few-shot and chain-of-thoughts prompt architecture, thus avoiding the additional costs of fine-tuning the model and maintaining it.
% % OpenAI offers an online solution to which we can make API calls to use the off-the-shelf model. 
% % Such approach has the advantage of not requiring hosting the LLMs, but also to explore the most recent advances in GPT models as they come out. 
% In future work, we consider exploring fine-tuning the model, which could lead to better feedback as the LLM would be aware of review practices for the specific targeted organizations.
% We would evaluate the relevancy of fine-tuning, regarding the trade-off between the improvement on comment generation and the related extra costs, either monetary when using an online solution, or computational and storage cost when hosting the model.


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/7-threats.tex <==
% Our study has threats to validity that might impact our results. Below, we discuss some of them in detail.

\emph{\textbf{Construct to Validity:}} 
\toolName\ currently is limited to two RAG approaches, one retrieving extra code context, the other relevant examples of past chunks with their review comment. 
Although other approaches could be explored, we chose those two
% , as well as other architecture choices (e.g., LLM-as-a-Judge, chain-of-thought), 
to cover a wider range of modern LLM techniques currently applied in the SE domain~\cite{zhou2022docprompting, parvez2021retrieval}.

% When evaluating the frequency of generated comments being accepted by reviewers, we may miss some cases as reviewers could reject the comment but still use its content. 
% The opposite scenario can also occur, as developers might accept comments but later change the content posted partially or entirely. 
% To minimize this threat, we further compare the contents of comments posted and rejected; \lm{Finish based on the results}

% Although engagement covers different aspects involving social and technical skills, in our investigation, we focus only on the responsiveness of developers, specifically the number of interactions (replies) from a given comment. 
% We do not assess the content of these interactions; however, we expect that replies directly posted for a given comment still address the previous comment issue. 
% In the same way, since we expect \toolName\ to generate concise comments, the number of replies asking for clarifications may decrease compared to comments exclusively generated by humans. 

% Regarding assessing the impact on productivity, we focus exclusively on the speed at which reviewers provide code reviews after the initial assignment and how fast developers send new patches addressing the reported code review. 
% Regarding the provided code reviews, knowing that different factors might influence our results, like developer's experience, time zone, and system knowledge, we try to address such a threat by selecting experienced participants who actively work on the projects targeted by \toolName.
% We do not evaluate the content of new patches sent by developers to address review comments, as we consider the time interval between these two events in our analysis.
% However, if a revision is accepted, we assume the contribution was properly further evaluated by reviewers, following the good practices and quality established for the project.




\emph{\textbf{Internal Validity:}} 
% Over time, reviewers might get used to \toolName, possibly influencing their acceptance or rejection independently of the comments' quality. 
% However, as different patches are associated with supporting code, when applicable, we expect the comments to address different aspects, which reviewers might further check. 
Reviewers might accept or reject comments based on their personal judgment and/or style of reviews. 
% For instance, they might prioritize comments addressing issues/bugs in the code under analysis, instead of also considering comments on documentation and code organization.
When evaluating productivity, different factors, like deadlines, policies, preferences, and tool changes, might affect our results, which we cannot control during our investigation. 

% \st{When classifying the categories of generated comments in RQ2, we perform a manual analysis evaluating their content.
% In this study, two researchers perform their individual analyses and later compare their reports with each other; the agreement was almost perfect, and imminent conflicts were discussed together, reaching a final consensus or rejection of the comment.} \bram{wasn't there one qualitative study where agreement was 0.45?}\Do{true, rephrasing the all paragraph to focus on the issue with the LLM labelling} \st{
% To mitigate associated biases with personal judgment, we adopted a pre-defined list of categories, guiding the researchers when classifying the comments.}
When classifying the categories of generated comments in RQ2, we perform an automated labelling using LLM.
To mitigate the potential hallucination of the model, we compared the automated labelling with a ground truth build through manual labelling.
% In the construction of the ground truth, two researchers perform their individual analyses and later compare their reports with each other; the agreement was almost perfect, and imminent conflicts were discussed together, reaching a final consensus or rejection of the comment. 
% To mitigate associated biases with personal judgment, we adopted a pre-defined list of categories~\cite{turzo2024makes}, guiding the researchers when classifying the comments.
The LLM was provided with a few-shot list of categories~\cite{turzo2024makes}. 
When compared with the ground truth, the automated labelling reached a moderate agreement with the ground truth, i.e., we observed no substantial hallucination.




\emph{\textbf{External Validity:}} Exploring review comment generation for other organizations might impact results based on their review policies and practices.
However, our investigation covers two organizations, one being open-source, and one closed-source. Despite their differences, we found that the two organizations achieved similar results in the user study. 



\toolName\ generates comments based on OpenAI's GPT4o.
LLMs are known to be computationally expensive, regarding both training and generations.
The approach we consider uses an off-the-shelf model with few-shot and chain-of-thoughts prompt architecture, thus avoiding the additional costs of fine-tuning the model and maintaining it.
% OpenAI offers an online solution to which we can make API calls to use the off-the-shelf model. 
% Such approach has the advantage of not requiring hosting the LLMs, but also to explore the most recent advances in GPT models as they come out. 
Future work should consider exploring fine-tuning the model, %, which could lead to better feedback as the LLM would be better aware of review practices for the specific targeted organizations.
% Such study would evaluate 
regarding the trade-off between the improvement on comment generation and the related extra costs (e.g., computational effort). %, either monetary when using an online solution, or computational and storage costs when hosting the model, which was outside of the scope of this study.


% Our results are also restricted to patches no larger than 3000 tokens; evaluating \toolName\ with larger patches is worth investigating, considering the diversity of code contributions requiring code reviews. 


% \begin{comment}
%     \item Although developers can disapprove comments, they can still use previously disapproved comments and post them as originally and exclusively created by them, without any support. What if we compute all generated comments and later check the similarity with the posted ones?
%     \item Developers can accept comments without properly evaluating the contents. What if we compute the time of (I) generated and (ii) posted code review comments? 
%     \item Different time zones might impact our metrics regarding timing and productivity.
% \end{comment}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/9-conclusion.tex <==

Code review plays an essential role in modern collaborative software development, representing a way to improve the quality of evolving systems while improving developers' social and technical skills~\cite{mcintosh2016empirical}. 
Recent studies have introduced review comment generation tasks into the review process, enhanced by LLM-based approaches~\cite{tufano2022using, li2022automating}.
However, they have not evaluated the impact of such approaches on the review process.

Through a large-scale mixed open-/closed-source user study, we report acceptance ratios of 8.1\% for Mozilla and 7.2\% for Ubisoft, and we further observe that appreciation is higher (23\% and 28.3\%, respectively). 
Refactoring comments, despite being the second most popular type of generated comments (15.8\% and 14.5\%) after functional comments (79.2\% and 84.8\%), have significantly better acceptance levels (18.2\% vs 4.8\% and 18.6\% vs 5.2\%).
The impact of the LLM-based approach on the review workflow is reasonable as reviewers spend a median time of 43s per review on investigating generated comments and, when applicable, editing accepted ones (37/119) to, in most cases, shorten them (25/37).
Regarding accepted comments, we find that their impact on patches’ review processes is similar to human-written comments, as 74\% vs 73\% of comments have at least one follow-up revision at chunk-level, which is promising for future adoption of LLM-generated review comments.

We hypothesize that the gap between acceptance and appreciation of generated review comments stems from the task not being properly defined for the LLM. 
Indeed, the LLM involved addresses multiple tasks, i.e., generating publishable comments, tips for developers and tips for reviewers, all of those being valuable to the review process.
We conclude that the current way of generating and presenting the results of review comment generation to reviewers and patch authors in the review environment should be reconsidered.% is not optimal compared to their purpose, as some comments should be shown to the developers prior to the review process (in the development phase) or shown as reviewer tips, not as an actual publishable comment. 
%We also argue that different categories of comments could be considered as a separate task, and could be split as well or at least evaluated separately.
% Future work should focus on splitting those tasks, as well as improving the relevancy of comments, as many are still marked as invalid, trivial, or too long. 
%\Do{need to be more vague according to Sarra because future work. I "vagified" the paragraph, let me know what you think}\bram{I commented out even more}


% Modern code review plays an essential approach in modern collaborative software development, representing a way to improve the quality of evolving systems while improving developers' social and technical skills~\cite{mcintosh2016empirical}. 
% However, performing good code reviews is costly, as it requires developers with advanced skills and impacts the team's productivity~\cite{tufano2021towards}.
% Research has been done to support developers in performing such tasks~\cite{tufano2022using, li2022automating}. %; however, their results are still limited to human intervention.
% With the advances of LLMs and their power to perform NLP tasks, researchers have investigated the feasibility of using these models to perform code reviews automatically; however, they miss proper evaluation in real context~\cite{tufano2024code}.
% To address this gap, in this paper, we conduct a user study in two companies with our prototype, \toolName, an LLM-based assistive tool for code reviews.
% To evaluate the impact of review comment generation, we perform an empirical evaluation with expert reviewers using the \toolName\ integrated into their review tool, during their day-to-day tasks.

% Our results report acceptance ratios of 8.1\% for Organization1 and 7.2\% for Organization2.
% Furthermore, we observe that respectively to each Organization, 32.2 and 20.3\% of generated comments, although not usable as comments, still bring potential value as either a tip for the reviewer, or a valid development tip, which should have been shown to the author of the patch prior to code submission. 
% Such valuable suggestions contribute to the value of the LLM-based review comment generation, in addition to the accepted comments, thus reporting an overall appreciation ratio between 20.3-32.2\%.
% Then, we studied the type of comments that are suggested, noticing that the most common type is functional comments (83-84\%).
% Refactoring comments, although being the second most popular type of comments (12-17\%), is significantly more accepted (18.8\% for Company1 and 18.9\% for Company2 compared to 4.9 and 5.1\% respectively).

% Regarding the additional effort needed when using the LLM-based approach, users spent a median time per patch of 43s dedicated to the suggestion inspection, which is an acceptable time dedication as most users reported that the extra time was only longer (24/37 users). 
% For accepted comment suggestions, reviewers usually spent a longer time than for rejected ones (median of 27.6s compared to 16s) which is due to verifying the validity of the comment and potential edits. We found that users report the comments to be often to wordy, which lead to shortening 24/117 accepted comments.

% Finally, we found that accepted comment suggestions lead to the same ratio of revision as human comments (74\% compared to 73\%), though the suggestions lead to significantly fewer threads (23\% compared to 34\%), as expected,  since the purpose of the suggestions were not to start discussions.

% Future work should explore improving acceptance ratios by filtering the potential impact of comments, where some suggested comments can be used as-is, but others should be displayed as warnings (review tips) or altogether shown prior to the review process (development tip). 
% Furthermore, as the review task is quite personal to individuals’ taste, exploring customization to better fulfill users’ needs would improve the impact and appreciation of such tool.

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/sections/our_settings.tex <==
\newboolean{showcomments}
\setboolean{showcomments}{true}
% \setboolean{showcomments}{false}
% \ifthenelse{\boolean{showcomments}}
%  { \newcommand{\mynote}[2]{
%       \fbox{\bfseries\sffamily\scriptsize#1}
%         {\small$\blacktriangleright$\textsf{\emph{#2}}$\blacktriangleleft$}}}
% { \newcommand{\mynote}[2]{}}
\ifthenelse{\boolean{showcomments}}
 { \newcommand{\mynote}[2]{
      \fbox{\bfseries\sffamily\scriptsize#1}
        $[$#2$]$}}
{ \newcommand{\mynote}[2]{}
}

\ifthenelse{\boolean{showcomments}}
 { \newcommand{\fixes}[2]{\textcolor{red}{\st{#1}} \textcolor{blue}{#2}}
 }
{ 
\newcommand{\fixes}[2]{#2}
}



\newcommand{\toolName}{RevMate}
\newcommand{\sm}[1]{\textcolor{red}{\mynote{Suhaib}{#1}}}
\newcommand{\lm}[1]{\textcolor{blue}{\mynote{Leuson}{#1}}}
\newcommand{\mc}[1]{\textcolor{green}{\mynote{Marco}{#1}}}
\newcommand{\Foutse}[1]{\textcolor{purple}{\mynote{Foutse}{#1}}}
\newcommand{\Do}[1]{\textcolor{red}{\mynote{Doriane}{#1}}}
\newcommand{\sh}[1]{\textcolor{orange}{\mynote{Sarra}{#1}}}
\newcommand{\bram}[1]{\textcolor{orange}{\mynote{Bram}{#1}}}


% \newcommand{\fixes}[2]{\textcolor{red}{\st{#1}} \textcolor{blue}{#2}}
% % \newcommand{\fixes}[2]{#2}
\usepackage[linesnumbered,vlined,ruled,boxed,commentsnumbered]{algorithm2e}
% \usepackage{listings}
\usepackage{xcolor}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{tabularx}
\usepackage{diagbox}
\usepackage{multirow}
\usepackage{hyperref}

\usepackage{fancybox}
\usepackage{soul}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Throw}{throw}{}{}


\newcommand{\suggRQone}{How frequently do reviewers accept comments generated by an LLM-based approach?}
\newcommand{\suggRQtwo}{How does the comment category correlate with acceptance ratios?}
\newcommand{\suggRQthree}{How does the adoption of LLM-generated comments impact the code review workflow?}
\newcommand{\suggRQfour}{How does the adoption of LLM-generated comments impact the patch's review process?}
% \newcommand{\suggRQfive}{What is the type of edits reviewer do to \toolName’s suggestions, if any?}



\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/prompts.tex <==
\begin{table*}[t]
    \centering
    \caption{Prompts and conversation used by \toolName}
    \label{tab:prompts}
    \begin{tabularx}{\textwidth}{|X|}
    \hline
\textbf{(1) Summary prompt (\textit{askLLMforSummary}):} \\\hline
    You are an expert reviewer for source code, with experience in source code reviews.
    Please, analyze the code provided and report a summarization about the new changes; for that, focus on the code added represented by lines that start with "+". \newline
    \textit{\{patch\}}\\
    \hline
    
\textbf{(2) Function request prompt (\textit{askLLMNeedsFuncs}):} \\\hline
Based on the patch provided below and its related summarization, identify the functions you need to examine for reviewing the patch.
List the names of these functions, providing only the function names, with each name on a separate line.
Avoid using list indicators such as hyphens or numbers.
If no function declaration is required, just return "".\newline
\textit{\{patch\}}
\textit{\{summarization\}} \\ \hline

\textbf{(3) Line context request prompt (\textit{askLLMNeedsLines}):} \\\hline
Based on the patch provided below and its related summarization, report the code lines for which more context is required.
For that, list the lines with their associated line numbers, grouping each one on a separate line.
Avoid using list indicators such as hyphens or numbers. If no code line is required, just return "".
Examples of valid code lines: '152    const selector = notification.getDescription();' and '56        file.getElement(this.targetElement());'\newline
\textit{\{patch\}}
\textit{\{summarization\}}\\\hline

\textbf{(4) Memory conversation content (\textit{memory}):} \\ \hline

\textbf{in:} You are an expert reviewer for source code, with experience on source code reviews.\newline 
\textbf{out:} Sure, I'm aware of source code practices in the development community. \newline
\textbf{in:} Please, analyze the code provided and report a summarization about the new changes; for that, focus on the code added represented by lines that start with "+". \textit{\{patch\}}\newline
\textbf{out:} \textit{\{summarization\}}\newline
if requested context: \newline 
\textbf{in:} Attached, you can find some function definitions that are used in the current patch and might be useful to you, by giving more context about the code under analysis.
\textit{\{function context\}}\newline
\textbf{out:} Okay, I will consider the provided function definitions as additional context to the given patch.\newline
\textbf{in:} Attached, you can also have more context of the target code under analysis.
\textit{\{line context\}}\newline
\textbf{out:} Okay, I will also consider the code as additional context to the given patch.
\\\hline

\textbf{(5) Review generation prompt (\textit{askLLMReview}):} \\\hline
    You will be given a task to generate a code review for the patch below. Use the following steps to solve it:\newline
    1. Understand the changes done in the patch by reasoning about the summarization as previously reported.\newline
    2. Identify possible code snippets that might result in possible bugs, major readability regressions, and similar concerns.\newline
    3. Reason about each identified problem to make sure they are valid. Keep in mind, your review must be consistent with the source code.\newline
    4. Filter out comments that focus on documentation, comments, error handling, tests, and confirmation whether objects, methods and files exist or not.\newline
    5. Filter out comments that are descriptive and filter out comments that are praising (example: "This is a good addition to the code.").\newline
    6. Filter out comments that are not about added lines (have a '+' symbol at the start of the line).\newline
    7. Final answer: Write down the comments and report them using the JSON format previously adopted for the valid comment examples.\newline
    As valid comments, consider the examples below:
    \textit{\{ex\}}
    \newline
    Here is the patch that we need you to review:
    \textit{\{patch\}}\\ \hline


\textbf{(6) Review generation filtering prompt (\textit{askLLMFilter}):} \\\hline

Please, double check the code review provided for the patch below.
Just report the comments that are:\newline
- applicable for the patch;\newline
- consistent with the source code;\newline
- focusing on reporting possible bugs, major readability regressions, or similar concerns;\newline
- filter out any descriptive comments;\newline
- filter out any praising comments;\newline
- filter out any comments that do not suggest code changes.\newline
Do not change the contents of the comments and the report format.
Adopt the template below as the report format:\newline
[
    \{
        "file": "com/br/main/Pressure.java",
        "code\_line": 458,
        "comment" : "a generated comment"
    \}
]\newline
Do not report any explanation about your choice.\newline
Review:
\textit{\{review\}} -
Patch:
\textit{\{patch\}}\newline
As examples of unexpected comments, unrelated to the current patch, please, check some below: \textit{\{undesired\_comments\}}\\ \hline
    \end{tabularx}
\end{table*}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq1_eval.tex <==



% \begin{table*}[h]
%     \centering
%     \caption{RQ1 - Evaluation counts (OLD VERSION)}
%     \label{tab:rq1eval}
%     \begin{tabularx}{\textwidth}{l|l||XXX|X||XX|X}
%     \hline
%          \textbf{Macro-}& \multirow{3}{*}{\textbf{Evaluation}}& \multicolumn{4}{c||}{\textbf{Open-source}}& \multicolumn{3}{c}{\textbf{Closed-source}} \\
%          \textbf{Evaluation}&&\multicolumn{3}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}\\
%           &&Code&Example&Combi&&Code&Example&\\
%          \hline

% \hline \multirow{1}{*}{Accepted} & Accept & 5 (7\%) & 19 (10\%) & 5 (6\%) & 29 (9\%) & 31 (8\%) & 54 (13\%) & 85 (11\%) \\
% \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a review tip & / & / & / & / & 51 (13\%) & 43 (10\%) & 94 (12\%) \\
%  & Ignore - Useful for developer & 4 (5\%) & 6 (3\%) & 1 (1\%) & 11 (3\%) & 105 (28\%) & 51 (12\%) & 156 (19\%) \\
% \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 29 (40\%) & 80 (43\%) & 31 (37\%) & 140 (41\%) & 112 (29\%) & 66 (15\%) & 178 (22\%) \\
%  & Ignore - Incorrect comment & 29 (40\%) & 65 (35\%) & 46 (55\%) & 140 (41\%) & 47 (12\%) & 137 (32\%) & 184 (23\%) \\
%  & Ignore - Other & 5 (7\%) & 12 (7\%) & / & 17 (5\%) & 28 (7\%) & 50 (12\%) & 78 (10\%) \\
% \hline \textit{Filter out}  & Ignore - I'm not sure & 1 (1\%) & 2 (1\%) & / & 3 (1\%) & 6 (2\%) & 27 (6\%) & 33 (4\%) \\
% \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
%  & 73 & 184 & 83 & 340 & 380 & 428 & 808 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
%  & 10 & 15 & 13 & 19 & 15 & 11 & 26 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
%  & 35 & 61 & 32 & 128 & 131 & 156 & 286 \\
%      \end{tabularx}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{RQ1 - Evaluation counts. ``Total" refers to the union of all the generated comments, disregarding the approach used.}
    \label{tab:rq1eval}
    \begin{tabularx}{\textwidth}{l|l||XX|X||XX|X}
    \hline
         \textbf{Macro-}& \multirow{3}{*}{\textbf{Evaluation}}& \multicolumn{3}{c||}{\textbf{Mozilla}}& \multicolumn{3}{c}{\textbf{Ubisoft}} \\
         \textbf{Evaluation}&&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}\\
          &&Code&Example&&Code&Example&\\
         \hline

% \hline \multirow{1}{*}{Accepted} & Accept & 8 (6\%) & 24 (9\%) & 32 (8\%) & 31 (5\%) & 54 (9\%) & 85 (7\%) \\
% \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & 19 (15\%) & 19 (7\%) & 38 (10\%) & 51 (9\%) & 43 (7\%) & 94 (8\%) \\
%  & Ignore - Useful for developer & 10 (8\%) & 12 (4\%) & 22 (6\%) & 105 (18\%) & 51 (8\%) & 156 (13\%) \\
% \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 36 (29\%) & 110 (40\%) & 146 (36\%) & 112 (19\%) & 66 (10\%) & 178 (15\%) \\
%  & Ignore - Incorrect comment & 40 (32\%) & 87 (32\%) & 127 (32\%) & 47 (8\%) & 137 (22\%) & 184 (15\%) \\
%  & Ignore - Other & 9 (7\%) & 19 (7\%) & 28 (7\%) & 28 (5\%) & 50 (8\%) & 78 (6\%) \\
%  & Ignore - Seen & / & / & / & 206 (35\%) & 204 (32\%) & 410 (34\%) \\
%  \hline \textit{Filter out}  & Ignore - I'm not sure & 4 (3\%) & 3 (1\%) & 7 (2\%) & 6 (1\%) & 27 (4\%) & 33 (3\%) \\
% \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
%  & 126 & 274 & 400 & 586 & 632 & 1218 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
%  & 18 & 21 & 26 & 17 & 14 & 31 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
%  & 55 & 96 & 151 & 197 & 227 & 422 \\

% \hline \multirow{1}{*}{Accepted} & Accept & 8 (6\%) & 24 (9\%) & 32 (8\%) & 31 (5\%) & 54 (9\%) & 85 (7\%) \\
% \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & 19 (15\%) & 19 (7\%) & 38 (10\%) & 51 (9\%) & 43 (7\%) & 94 (8\%) \\
%  & Ignore - Useful for developer & 10 (8\%) & 12 (4\%) & 22 (6\%) & 105 (18\%) & 51 (8\%) & 156 (13\%) \\
% \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 36 (29\%) & 110 (40\%) & 146 (36\%) & 112 (19\%) & 66 (10\%) & 178 (15\%) \\
%  & Ignore - Incorrect comment & 40 (32\%) & 87 (32\%) & 127 (32\%) & 47 (8\%) & 137 (22\%) & 184 (15\%) \\
%  & Ignore - Other & 9 (7\%) & 19 (7\%) & 28 (7\%) & 28 (5\%) & 50 (8\%) & 78 (6\%) \\
%  & Ignore - None & / & / & / & 206 (35\%) & 204 (32\%) & 410 (34\%) \\
% \hline \textit{Filter out} & Ignore - I'm not sure & 4 (3\%) & 3 (1\%) & 7 (2\%) & 6 (1\%) & 27 (4\%) & 33 (3\%) \\
% \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
%  & 126 & 274 & 400 & 586 & 632 & 1218 \\
% \multicolumn{2}{r|}{\textbf{Total \#evaluated}}% &
%  & 122 & 271 & 393 & 580 & 605 & 1185 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
%  & 18 & 21 & 26 & 17 & 14 & 31 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
%  & 55 & 96 & 151 & 197 & 227 & 422 \\


%  \hline \multirow{1}{*}{Accepted} & Accept & 8 (6.3\%) & 24 (8.8\%) & 32 (8.0\%) & 31 (5.3\%) & 54 (8.5\%) & 85 (7.0\%) \\
% \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & 19 (15.1\%) & 19 (6.9\%) & 38 (9.5\%) & 51 (8.7\%) & 43 (6.8\%) & 94 (7.7\%) \\
%  & Ignore - Useful for developer & 10 (7.9\%) & 12 (4.4\%) & 22 (5.5\%) & 105 (17.9\%) & 51 (8.1\%) & 156 (12.8\%) \\
% \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 36 (28.6\%) & 110 (40.1\%) & 146 (36.5\%) & 112 (19.1\%) & 66 (10.4\%) & 178 (14.6\%) \\
%  & Ignore - Incorrect comment & 40 (31.7\%) & 87 (31.8\%) & 127 (31.8\%) & 47 (8.0\%) & 137 (21.7\%) & 184 (15.1\%) \\
%  & Ignore - Other & 9 (7.1\%) & 19 (6.9\%) & 28 (7.0\%) & 28 (4.8\%) & 50 (7.9\%) & 78 (6.4\%) \\
%  & Ignore - Seen & / & / & / & 206 (35.2\%) & 204 (32.3\%) & 410 (33.7\%) \\
% \hline \textit{Filter out} & Ignore - I'm not sure & 4 (3.2\%) & 3 (1.1\%) & 7 (1.8\%) & 6 (1.0\%) & 27 (4.3\%) & 33 (2.7\%) \\
% \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
%  & 126 & 274 & 400 & 586 & 632 & 1218 \\
%  \multicolumn{2}{r|}{\textbf{Total \#evaluated}}% &
%  & 122 & 271 & 393 & 580 & 605 & 1185 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
%  & 18 & 21 & 26 & 17 & 14 & 31 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
%  & 55 & 96 & 151 & 197 & 227 & 422 \\
 
\hline \multirow{1}{*}{Accepted} & Accept & 9 (6.8\%) & 25 (8.5\%) & 34 (8.0\%) & 31 (5.3\%) & 54 (8.5\%) & 85 (7.0\%) \\
\hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & 19 (14.4\%) & 20 (6.8\%) & 39 (9.2\%) & 51 (8.7\%) & 43 (6.8\%) & 94 (7.7\%) \\
 & Ignore - Useful for developer & 10 (7.6\%) & 13 (4.4\%) & 23 (5.4\%) & 105 (17.9\%) & 51 (8.1\%) & 156 (12.8\%) \\
\hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 37 (28.0\%) & 114 (38.8\%) & 151 (35.4\%) & 112 (19.1\%) & 66 (10.4\%) & 178 (14.6\%) \\
 & Ignore - Incorrect comment & 42 (31.8\%) & 100 (34.0\%) & 142 (33.3\%) & 47 (8.0\%) & 137 (21.7\%) & 184 (15.1\%) \\
 & Ignore - Other & 10 (7.6\%) & 19 (6.5\%) & 29 (6.8\%) & 28 (4.8\%) & 50 (7.9\%) & 78 (6.4\%) \\
 & Ignore - Seen & / & / & / & 206 (35.2\%) & 204 (32.3\%) & 410 (33.7\%) \\
 \hline \textit{Filter out} & Ignore - I'm not sure & 5 (3.8\%) & 3 (1.0\%) & 8 (1.9\%) & 6 (1.0\%) & 27 (4.3\%) & 33 (2.7\%) \\
\hline \hline \multicolumn{2}{r||}{\textbf{Total \#comments}}% &
 & 132 & 294 & 426 & 586 & 632 & 1218 \\
 \multicolumn{2}{r||}{\textbf{Total \#evaluated}}% &
 & 127 & 291 & 418 & 580 & 605 & 1185 \\
\multicolumn{2}{r||}{\textbf{Total \#reviewers}}% &
 & 19 & 22 & 28 & 17 & 14 & 31 \\
\multicolumn{2}{r||}{\textbf{Total \#reviews}}% &
 & 59 & 106 & 165 & 197 & 227 & 422 \\
 
     \end{tabularx}
\end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{RQ1 - Evaluation rates}
%     \label{tab:rq1eval}
%     \begin{tabularx}{\textwidth}{l|l|X|X|X|X}
%     \hline
%          \textbf{Macro-}& \multirow{2}{*}{\textbf{Evaluation}}& \multicolumn{2}{c|}{\textbf{Open-source}}& \multicolumn{2}{c}{\textbf{Closed-source}} \\
%          \textbf{Evaluation}&&\textbf{Code}&\textbf{Example}&\textbf{Code}&\textbf{Example}\\
%          \hline\hline
%          % \textbf{Accepted}&/&Positive&\\ \hline
%          % \multirow{6}{*}{\textbf{Ignored}} & Useful as review tip&Positive&\\\cline{2-4}
%          %  & Useful at development phase&Positive&\\\cline{2-4}
%          % &Trivial comment&Negative&\\\cline{2-4}
%          % &Invalid comment&Negative&\\\cline{2-4}
%          % &Other&Negative&\\\cline{2-4}
%          % & I'm not sure&Neutral&\\\cline{2-4}

% % \hline \multirow{1}{*}{Accepted} & Accept & NaN & NaN & 21 (8\%) & 49 (13\%) \\
% % \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & NaN & NaN & 36 (14\%) & 43 (11\%) \\
% %  & Ignore - Useful for developer & NaN & NaN & 72 (28\%) & 34 (9\%) \\
% % \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & NaN & NaN & 68 (26\%) & 56 (15\%) \\
% %  & Ignore - Incorrect comment & NaN & NaN & 32 (12\%) & 121 (32\%) \\
% %  & Ignore - Other & NaN & NaN & 25 (10\%) & 47 (12\%) \\
% % \hline \multirow{1}{*}{\textit{Filter out}} & Ignore - I'm not sure & NaN & NaN & 3 (1\%) & 27 (7\%) \\
% % \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
% %  & NaN & NaN & 257 & 377 \\
% % \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
% %  & NaN & NaN & 10 & 11 \\
% % \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
% %  & NaN & NaN & 90 & 136 \\

% \hline \multirow{1}{*}{Accepted} & Accept & 5 (7\%) & 19 (10\%) & 31 (8\%) & 54 (13\%) \\
% \hline \multirow{1}{*}{Valuable Tip} & Ignore - Useful as a tip for reviewers & NaN & NaN & 51 (13\%) & 43 (10\%) \\
%  & Ignore - Useful for developer & 4 (5\%) & 6 (3\%) & 105 (28\%) & 51 (12\%) \\
% \hline \multirow{1}{*}{Rejected} & Ignore - Trivial comment & 29 (40\%) & 80 (43\%) & 112 (29\%) & 66 (15\%) \\
%  & Ignore - Incorrect comment & 29 (40\%) & 65 (35\%) & 47 (12\%) & 137 (32\%) \\
%  & Ignore - Other & 5 (7\%) & 12 (7\%) & 28 (7\%) & 50 (12\%) \\
%  & Ignore - I'm not sure & 1 (1\%) & 2 (1\%) & 6 (2\%) & 27 (6\%) \\
% \hline \hline \multicolumn{2}{r|}{\textbf{Total \#comments}}% &
%  & 73 & 184 & 380 & 428 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviewers}}% &
%  & 10 & 15 & 15 & 11 \\
% \multicolumn{2}{r|}{\textbf{Total \#reviews}}% &
%  & 35 & 61 & 131 & 156 \\
%     \end{tabularx}
% \end{table*}



==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq1_res.tex <==
% \begin{table}[h]
%     \centering
%     \caption{RQ1\&2 - Evaluation rates}
%     \label{tab:rq1res}
%     \begin{tabularx}{\linewidth}{l||XXX|X||XX|X}
%     \hline
%          \textbf{Rates}& \multicolumn{4}{c||}{\textbf{Open-source}}& \multicolumn{3}{c}{\textbf{Closed-source}} \\
%          \textbf{[\%]}&\multicolumn{3}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}\\
%           &Code&Ex&Comb&&Code&Ex&\\
%          \hline
% % All\\
% % Acceptance & 6.9 & 10.4 & 6.0 & 8.6 & 8.3 & 13.5 & 11.0 \\
% % Appreciation & 12.5 & 13.7 & 7.2 & 11.9 & 50.0 & 36.9 & 43.2 \\
% % \hline

% % Functional\\% &
% %  Acceptance & NaN & NaN & NaN & NaN & 5.4 & 9.6 & 7.4 \\
% % % &
% %  Appreciation & NaN & NaN & NaN & NaN & 47.2 & 35.0 & 40.9 \\
% % \hline Refactoring\\% &
% %  Acceptance & NaN & NaN & NaN & NaN & 19.4 & 29.5 & 25.0 \\
% % % &
% %  Appreciation & NaN & NaN & NaN & NaN & 50.6 & 48.2 & 49.8 \\
% % \hline Documentation\\% &
% %  Acceptance & NaN & NaN & NaN & NaN & 0.0 & NaN & 0.0 \\
% % % &
% %  Appreciation & NaN & NaN & NaN & NaN & 100.0 & NaN & 100.0 \\
% % \hline Discussion\\% &
% %  Acceptance & NaN & NaN & NaN & NaN & 10.4 & 0.0 & 4.1 \\
% % % &
% %  Appreciation & NaN & NaN & NaN & NaN & 75.4 & 21.3 & 43.3 \\


% \hline\hline 
% All\\
% Acceptance [\%] & 6.6 & 8.9 & 8.1 & 5.3 & 8.9 & 7.2 \\
% Appreciation [\%] & 30.3 & 20.3 & 23.4 & 32.2 & 24.5 & 28.3 \\
% \hline
% Functional\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 3.4 & 6.3 & 4.8 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 29.8 & 22.9 & 26.3 \\
% \hline Refactoring\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 12.6 & 20.8 & 17.0 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 32.7 & 34.0 & 33.9 \\
%  \end{tabularx}
% \end{table}


\begin{table}[t]
    \centering
    \caption{RQ1- Evaluation ratios. ``Total" refers to the union of all the generated comments, disregarding the approach used.}
    \label{tab:rq1res}
    \begin{tabularx}{\linewidth}{l||XX|X||XX|X}
    \hline
         & \multicolumn{3}{c||}{\textbf{Mozilla}}& \multicolumn{3}{c}{\textbf{Ubisoft}} \\
         \textbf{Ratio}&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}&\multicolumn{2}{c|}{\textbf{Approach}}&\multirow{2}{*}{\textbf{Total}}\\
          &Code&Ex&&Code&Ex&\\
         \hline
% All\\
% Acceptance & 6.9 & 10.4 & 6.0 & 8.6 & 8.3 & 13.5 & 11.0 \\
% Appreciation & 12.5 & 13.7 & 7.2 & 11.9 & 50.0 & 36.9 & 43.2 \\
% \hline

% Functional\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 5.4 & 9.6 & 7.4 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 47.2 & 35.0 & 40.9 \\
% \hline Refactoring\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 19.4 & 29.5 & 25.0 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 50.6 & 48.2 & 49.8 \\
% \hline Documentation\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 0.0 & NaN & 0.0 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 100.0 & NaN & 100.0 \\
% \hline Discussion\\% &
%  Acceptance & NaN & NaN & NaN & NaN & 10.4 & 0.0 & 4.1 \\
% % &
%  Appreciation & NaN & NaN & NaN & NaN & 75.4 & 21.3 & 43.3 \\


\hline 

% All\\Acceptance [\%] & 6.6 & 8.9 & 8.1 & 5.3 & 8.9 & 7.2 \\
% Appreciation [\%] & 30.3 & 20.3 & 23.4 & 32.2 & 24.5 & 28.3 \\
% \hline Functional\\Acceptance [\%] & 3.0 & 5.8 & 4.9 & 3.3 & 6.8 & 5.1 \\
% Appreciation [\%] & 28.7 & 18.3 & 21.5 & 31.8 & 24.0 & 27.9 \\
% \hline Refactoring\\Acceptance [\%] & 23.8 & 15.6 & 18.9 & 16.9 & 20.4 & 18.8 \\
% Appreciation [\%] & 38.1 & 21.9 & 28.3 & 33.7 & 27.6 & 30.4 \\


% \hline \textbf{All}&&&&&\\
Acceptance [\%] & 7.1 & 8.6 & 8.1 & 5.3 & 8.9 & 7.2 \\
Appreciation [\%] & 29.9 & 19.9 & 23.0 & 32.2 & 24.5 & 28.3 \\
\hline
% \hline\hline \textbf{Functional}&&&&&\\Acceptance [\%] & 4.1 & 5.1 & 4.8 & 4.0 & 6.3 & 5.2 \\
% Appreciation [\%] & 23.7 & 17.1 & 19.0 & 33.4 & 24.6 & 29.0 \\
% \hline \textbf{Refactoring}&&&&&\\Acceptance [\%] & 19.2 & 17.5 & 18.2 & 13.0 & 23.2 & 18.6 \\
% Appreciation [\%] & 57.7 & 22.5 & 36.4 & 24.7 & 25.3 & 25.0 \\

% \hline Documentation\\Acceptance [\%] & 0.0 & 100.0 & 75.0 & 0.0 & 25.0 & 20.0 \\
% Appreciation [\%] & 0.0 & 100.0 & 75.0 & 0.0 & 25.0 & 20.0 \\
% \hline Discussion\\Acceptance [\%] & 0.0 & 0.0 & 0.0 & NaN & 0.0 & 0.0 \\
% Appreciation [\%] & 0.0 & 37.5 & 27.3 & NaN & 33.3 & 33.3 \\

% Documentation\\Acceptance [\%] & 0.0 & 50.0 & 44.4 & 50.0 & 0.0 & 20.0 \\
% Appreciation [\%] & 0.0 & 50.0 & 44.4 & 50.0 & 0.0 & 20.0 \\
% Discussion\\Acceptance [\%] & NaN & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% Appreciation [\%] & NaN & 0.0 & 0.0 & 100.0 & 0.0 & 16.7 \\

% Functional\\% &
%  Acceptance & NaN & NaN  & NaN & 3.4 & 6.3 & 4.8 \\
% % &
%  Appreciation & NaN & NaN  & NaN & 29.8 & 22.9 & 26.3 \\
% \hline Refactoring\\% &
%  Acceptance & NaN & NaN  & NaN & 12.6 & 20.8 & 17.0 \\
% % &
%  Appreciation & NaN & NaN  & NaN & 32.7 & 34.0 & 33.9 \\
 \end{tabularx}
\end{table}

% \begin{table}[h]
%     \centering
%     \caption{RQ1\&2 - Evaluation rates}
%     \label{tab:rq1res}
%     \begin{tabularx}{\linewidth}{r|X|X|X|X}
%     \hline
%          \textbf{Rates}& \multicolumn{2}{c|}{\textbf{Open-source}}& \multicolumn{2}{c}{\textbf{Closed-source}} \\
%          &\textbf{Code}&\textbf{Example}&\textbf{Code}&\textbf{Example}\\
%          \hline\hline
% All &&&&\\
% Acceptance [\%] & 6.9 & 10.4 & 8.3 & 13.5 \\
% Appreciation [\%] & 12.5 & 13.7 & 50.0 & 36.9 \\
% \hline

% % Functional\\% &
% %  Acceptance [\%] & NaN & NaN & 7.3 & 7.4 \\
% % % &
% %  Appreciation [\%] & NaN & NaN & 49.4 & 35.4 \\
% % \hline Refactoring\\% &
% %  Acceptance [\%] & NaN & NaN & 12.2 & 30.9 \\
% % % &
% %  Appreciation [\%] & NaN & NaN & 52.1 & 46.7 \\
% % \hline Documentation\\% &
% %  Acceptance [\%] & NaN & NaN & NaN & NaN \\
% % % &
% %  Appreciation [\%] & NaN & NaN & NaN & NaN \\
% % \hline Discussion\\% &
% %  Acceptance [\%] & NaN & NaN & NaN & 0.0 \\
% % % &
% %  Appreciation [\%] & NaN & NaN & NaN & 19.9 \\

% Functional\\% &
%  Acceptance [\%] & NaN & NaN & 5.4 & 9.6 \\
% % &
%  Appreciation [\%] & NaN & NaN & 47.2 & 35.0 \\
% \hline Refactoring\\% &
%  Acceptance [\%] & NaN & NaN & 19.4 & 29.5 \\
% % &
%  Appreciation [\%] & NaN & NaN & 50.6 & 48.2 \\
% % \hline Documentation\\% &
% %  Acceptance [\%] & NaN & NaN & 0.0 & NaN \\
% % % &
% %  Appreciation [\%] & NaN & NaN & 100.0 & NaN \\
% % \hline Discussion\\% &
% %  Acceptance [\%] & NaN & NaN & 10.4 & 0.0 \\
% % % &
% %  Appreciation [\%] & NaN & NaN & 75.4 & 21.3 \\
 
%          \hline 
%     \end{tabularx}
% \end{table}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq1_stats.tex <==
\begin{table}[t]
    \caption{RQ1: Fisher's statistical test's p-values when comparing Organization1 to Organization2 given a specific evaluation set and a metric.}
    \label{tab:rq1stat}
    \centering
    \begin{tabularx}{\linewidth}{l|X|X|X}
        \hline
        \backslashbox{\textbf{Metric}}{\textbf{Evaluation set}}& \textbf{Code} & \textbf{Example} & \textbf{Total}  \\
        \hline
         \textbf{Acceptance}&.363&.559&.296\\
         \textbf{Appreciation}&.696&.926&.975\\
        \hline
    \end{tabularx}
    
\end{table}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq2_type.tex <==

% \begin{table}[h]
%     \centering
%     \caption{RQ2 - Impact of the type of comments}
%     \label{tab:rq2type}
%     \begin{tabularx}{.47\textwidth}{rr|X|X|X|X}
%     \hline
%          \textbf{Comment}&& \multicolumn{2}{c|}{\textbf{Open-source}}& \multicolumn{2}{c}{\textbf{Closed-source}} \\
%         \textbf{category}& &RAG-Context&RAG-Examples&RAG-Context&RAG-Examples\\
%          \hline\hline
        %  Functional 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    & 11  & 8  \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Refactoring 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Discussion 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        % Tip 
        %  &All &  &    &   &   \\
        %  &Accepted &  &    &   &   \\
        %  &Useful &  &    &   &   \\
        %  &Ignored &  &    &   &   \\
        % \hline
        
% Accept & All & 0 & 0 & 13 & 25 \\
%  & Functional & NaN & NaN & 9 & 8 \\
%  & Refactoring & NaN & NaN & 4 & 17 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 0 \\
% \hline Useful & All & 0 & 0 & 20 & 20 \\
%  & Functional & NaN & NaN & 16 & 14 \\
%  & Refactoring & NaN & NaN & 4 & 4 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 2 \\
% \hline Ignore & All & 0 & 0 & 20 & 20 \\
%  & Functional & NaN & NaN & 16 & 12 \\
%  & Refactoring & NaN & NaN & 4 & 5 \\
%  & Documentation & NaN & NaN & 0 & 0 \\
%  & Discussion & NaN & NaN & 0 & 3 \\

% All labeled & Accept & 0 & 0 & 13 & 25 \\
%  & Useful & 0 & 0 & 20 & 20 \\
%  & Ignore & 0 & 0 & 20 & 20 \\
% \hline Functional & Accept & NaN & NaN & 9 & 8 \\
%  & Useful & NaN & NaN & 16 & 14 \\
%  & Ignore & NaN & NaN & 16 & 12 \\
% \hline Refactoring & Accept & NaN & NaN & 4 & 17 \\
%  & Useful & NaN & NaN & 4 & 4 \\
%  & Ignore & NaN & NaN & 4 & 5 \\
% \hline Documentation & Accept & NaN & NaN & 0 & 0 \\
%  & Useful & NaN & NaN & 0 & 0 \\
%  & Ignore & NaN & NaN & 0 & 0 \\
% \hline Discussion & Accept & NaN & NaN & 0 & 0 \\
%  & Useful & NaN & NaN & 0 & 2 \\
%  & Ignore & NaN & NaN & 0 & 3 \\
%         \hline
%     \end{tabularx}
% \end{table}



% \begin{table}[h]
%     \centering
%     \caption{RQ2 - Group of comments. "Sam" columns show counts from the samples where "Reb" represent the percentage of the original dataset size, rebalanced based on the true distribution of macro-evaluation. }
%     \label{tab:rq2type}
%     \begin{tabularx}{\linewidth}{p{.8cm}l|XX|XX|XX|XX}
%     \hline
%          && \multicolumn{4}{c|}{\textbf{Open-source}}& \multicolumn{4}{c}{\textbf{Closed-source}} \\
%         & &\multicolumn{2}{c|}{\textbf{Code}}&\multicolumn{2}{c|}{\textbf{Example}}&\multicolumn{2}{c|}
%         {\textbf{Code}}&\multicolumn{2}{c}{\textbf{Example}}\\
%         &&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb\\
%          \hline



% % \hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 13 & 8\% & 25 & 13\% \\
% %  & Valuable Tip & 0 & 0\% & 0 & 0\% & 20 & 42\% & 20 & 23\% \\
% %  & Rejected & 0 & 0\% & 0 & 0\% & 20 & 50\% & 20 & 63\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 53 & 100\% & 65 & 100\% \\
% % \hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & 9 & 6\% & 8 & 4\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 16 & 33\% & 14 & 16\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 16 & 40\% & 12 & 38\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 41 & 79\% & 34 & 59\% \\
% % \hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & 4 & 3\% & 17 & 9\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 4 & 8\% & 4 & 5\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 4 & 10\% & 5 & 16\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 12 & 21\% & 26 & 30\% \\
% % \hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
% % \hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% %  & Valuable Tip & NaN & nan\% & NaN & nan\% & 0 & 0\% & 2 & 2\% \\
% %  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 3 & 9\% \\
% % \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 5 & 12\% \\


% \hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 29 & 8\% & 50 & 13\% \\
%  & Valuable Tip & 0 & 0\% & 0 & 0\% & 35 & 42\% & 37 & 23\% \\
%  & Rejected & 0 & 0\% & 0 & 0\% & 37 & 50\% & 36 & 63\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 101 & 100\% & 123 & 100\% \\
% \hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & 14 & 4\% & 24 & 6\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 26 & 31\% & 27 & 17\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 29 & 39\% & 25 & 44\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 69 & 74\% & 76 & 67\% \\
% \hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & 13 & 4\% & 26 & 7\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 5 & 6\% & 7 & 4\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 7 & 9\% & 7 & 12\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 25 & 19\% & 40 & 24\% \\
% \hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 1 & 1\% & 0 & 0\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 1 & 1\% & 0 & 0\% \\
% \hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & 2 & 1\% & 0 & 0\% \\
%  & Valuable Tip & NaN & nan\% & NaN & nan\% & 3 & 4\% & 3 & 2\% \\
%  & Rejected & NaN & nan\% & NaN & nan\% & 1 & 1\% & 4 & 7\% \\
% \cline{2-10}  & Total & 0 & 0\% & 0 & 0\% & 6 & 5\% & 7 & 9\% \\
%          \hline
%     \end{tabularx}
% \end{table}



\begin{table*}[t]
    \centering
    \caption{RQ2 - Group of comments. "Sam" columns show counts from the samples where "Reb" represent the percentage of the original dataset size, rebalanced based on the true distribution of macro-evaluation. }
    \label{tab:rq2type}
    \begin{tabularx}{\textwidth}{ll|XXXXXX|XX||XXXX|XX}
    \hline
         && \multicolumn{8}{c||}{\textbf{Open-source}}& \multicolumn{6}{c}{\textbf{Closed-source}} \\
         & &\multicolumn{6}{c|}{\textbf{Approach}}&&&\multicolumn{4}{c}{\textbf{Approach}}
&&\\
        & &\multicolumn{2}{c}{\textbf{Code}}&\multicolumn{2}{c}{\textbf{Example}}&\multicolumn{2}{c|}{\textbf{Both}}&\multicolumn{2}{c|}{\textbf{Total}}&\multicolumn{2}{c}
        {\textbf{Code}}&\multicolumn{2}{c|}{\textbf{Example}}&\multicolumn{2}{c}{\textbf{Total}}\\
        &&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb&Sam&Reb\\
         \hline
\hline \multirow{4}{*}{All} & Accepted & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 29 & 8\% & 50 & 13\% & 79 & 11\% \\
 & Valuable Tip & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 35 & 42\% & 37 & 23\% & 72 & 32\% \\
 & Rejected & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 37 & 50\% & 36 & 63\% & 73 & 57\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 101 & 100\% & 123 & 100\% & 224 & 100\% \\
\hline \multirow{4}{*}{Functional} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 14 & 4\% & 24 & 6\% & 38 & 5\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 26 & 31\% & 27 & 17\% & 53 & 24\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 29 & 39\% & 25 & 44\% & 54 & 42\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 69 & 74\% & 76 & 67\% & 145 & 71\% \\
\hline \multirow{4}{*}{Refactoring} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 13 & 4\% & 26 & 7\% & 39 & 5\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 5 & 6\% & 7 & 4\% & 12 & 5\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 7 & 9\% & 7 & 12\% & 14 & 11\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 25 & 19\% & 40 & 24\% & 65 & 22\% \\
\hline \multirow{4}{*}{Documentation} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 1 & 1\% & 0 & 0\% & 1 & 0\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 0 & 0\% & 0 & 0\% & 0 & 0\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 1 & 1\% & 0 & 0\% & 1 & 0\% \\
\hline \multirow{4}{*}{Discussion} & Accepted & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 2 & 1\% & 0 & 0\% & 2 & 0\% \\
 & Valuable Tip & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 3 & 4\% & 3 & 2\% & 6 & 3\% \\
 & Rejected & NaN & nan\% & NaN & nan\% & NaN & nan\% & NaN & nan\% & 1 & 1\% & 4 & 7\% & 5 & 4\% \\
\cline{2-16}  & Total & 0 & 0\% & 0 & 0\% & 0 & 0\% & 0 & 0\% & 6 & 5\% & 7 & 9\% & 13 & 7\% \\

    \end{tabularx}
\end{table*}

==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq2_type_auto.tex <==

% \begin{table*}[h]
%     \centering
%     \caption{RQ2 - Type automatically generated }
%     \label{tab:rq2type}
%     \begin{tabularx}{\textwidth}{p{5cm}|XXX|XXX||XXX||XXX|XXX||XXX}
%     \hline
%          & \multicolumn{9}{c||}{\textbf{Open-source}}& \multicolumn{9}{c}{\textbf{Closed-source}} \\
%          &\multicolumn{6}{c||}{\textbf{Approach}}&&&&\multicolumn{6}{c||}{\textbf{Approach}}&&&\\
%         &\multicolumn{3}{c|}{\textbf{Code}}&\multicolumn{3}{c||}{\textbf{Example}}&\multicolumn{3}{c||}{\textbf{Total}}&\multicolumn{3}{c|}{\textbf{Code}}&\multicolumn{3}{c||}{\textbf{Example}}&\multicolumn{3}{c}{\textbf{Total}}\\
%         &Tot&Acc&App&Tot&Acc&App&Tot&Acc&App&Tot&Acc&App&Tot&Acc&App&Tot&Acc&App\\
%          \hline



% \textbf{CLUSTER K=5}\\\hline
% Code Quality and Safety Enhancements & 6 & 0\% & 17\% & 25 & 8\% & 8\% & 57 & 7\% & 11\% & 108 & 4\% & 25\% & 223 & 9\% & 23\% & 331 & 7\% & 24\% \\
% \hline
% Code Readability and Maintainability Improvements & 17 & 18\% & 24\% & 34 & 18\% & 18\% & 63 & 16\% & 17\% & 87 & 10\% & 22\% & 108 & 14\% & 24\% & 195 & 12\% & 23\% \\
% \hline
% Code Review and Refactoring Checklist & 49 & 4\% & 8\% & 117 & 9\% & 15\% & 207 & 7\% & 11\% & 69 & 4\% & 25\% & 67 & 13\% & 34\% & 136 & 9\% & 29\% \\
% \hline
% Code Review and Validation Checklist & - & - & - & 6 & 0\% & 0\% & 10 & 0\% & 0\% & 123 & 6\% & 44\% & 94 & 5\% & 13\% & 217 & 6\% & 30\% \\
% \hline
% Code Review: Null Checks, Error Handling, and Logic Validation & - & - & - & - & - & - & - & - & - & 193 & 4\% & 36\% & 113 & 4\% & 32\% & 306 & 4\% & 35\% \\


% \hline
% \textbf{CLUSTER K=8}\\\hline
% Code Refactoring and Validation Checklist & 8 & 0\% & 0\% & 59 & 3\% & 3\% & 71 & 3\% & 3\% & 7 & 0\% & 0\% & - & - & - & 7 & 0\% & 0\% \\
% \hline
% Code Quality and Maintenance Recommendations & 1 & 0\% & 0\% & 3 & 33\% & 33\% & 10 & 10\% & 10\% & 21 & 0\% & 24\% & 55 & 22\% & 33\% & 76 & 16\% & 30\% \\
% \hline
% Code Readability and Maintainability Improvements & 9 & 22\% & 33\% & 8 & 12\% & 12\% & 18 & 17\% & 22\% & 74 & 12\% & 27\% & 62 & 8\% & 21\% & 136 & 10\% & 24\% \\
% \hline
% Code Review and Quality Assurance Checklist & 3 & 0\% & 0\% & 13 & 0\% & 0\% & 26 & 0\% & 4\% & 127 & 4\% & 36\% & 132 & 9\% & 32\% & 259 & 7\% & 34\% \\
% \hline
% Code Review and Validation Checklist & - & - & - & 6 & 0\% & 0\% & 8 & 0\% & 0\% & 111 & 6\% & 38\% & 41 & 10\% & 27\% & 152 & 7\% & 35\% \\
% \hline
% Codebase Update and Validation Checklist & 9 & 0\% & 11\% & 3 & 0\% & 0\% & 18 & 0\% & 6\% & 93 & 0\% & 46\% & 104 & 2\% & 21\% & 197 & 1\% & 33\% \\
% \hline
% Null Pointer Dereference Risk Mitigations & 4 & 0\% & 25\% & 8 & 25\% & 25\% & 25 & 16\% & 20\% & 98 & 4\% & 19\% & 142 & 6\% & 18\% & 240 & 5\% & 19\% \\
% \hline
% Code Quality and Error Handling Improvements & 38 & 8\% & 11\% & 82 & 16\% & 23\% & 161 & 12\% & 16\% & 49 & 12\% & 24\% & 69 & 14\% & 23\% & 118 & 14\% & 24\% \\

% \hline 
% \textbf{CLUSTER K=10}\\\hline
% Code Quality and Consistency Improvements & 34 & 9\% & 12\% & 52 & 19\% & 23\% & 114 & 14\% & 17\% & 57 & 7\% & 25\% & 88 & 15\% & 32\% & 145 & 12\% & 29\% \\
% \hline
% Code Quality and Performance Improvement Suggestions & 3 & 0\% & 33\% & 19 & 16\% & 21\% & 29 & 14\% & 21\% & 54 & 6\% & 19\% & 51 & 12\% & 25\% & 105 & 9\% & 22\% \\
% \hline
% Code Quality and Validation Checklist & - & - & - & 6 & 0\% & 0\% & 9 & 0\% & 0\% & 98 & 7\% & 39\% & 66 & 11\% & 20\% & 164 & 9\% & 31\% \\
% \hline
% Code Readability and Maintainability Improvements & 9 & 22\% & 33\% & 8 & 12\% & 12\% & 22 & 14\% & 18\% & 51 & 12\% & 25\% & 52 & 10\% & 17\% & 103 & 11\% & 21\% \\
% \hline
% Code Review and Refactoring Checklist & 17 & 0\% & 0\% & 40 & 8\% & 15\% & 74 & 4\% & 8\% & 7 & 0\% & 0\% & - & - & - & 7 & 0\% & 0\% \\
% \hline
% Code Review and Validation Checklist & - & - & - & - & - & - & 1 & 0\% & 0\% & 148 & 5\% & 43\% & 74 & 3\% & 34\% & 222 & 4\% & 40\% \\
% \hline
% Code Review: Potential Issues and Best Practices for Robustness and Performance & 2 & 0\% & 0\% & 9 & 0\% & 0\% & 22 & 0\% & 5\% & 77 & 1\% & 32\% & 127 & 10\% & 31\% & 204 & 7\% & 31\% \\
% \hline
% Context-Specific Speed and Probe Update Validations & - & - & - & - & - & - & - & - & - & 9 & 0\% & 100\% & 24 & 0\% & 0\% & 33 & 0\% & 27\% \\
% \hline
% Initialization and Parameter Handling in Compilation and Instantiation Processes & 3 & 0\% & 0\% & 38 & 0\% & 0\% & 41 & 0\% & 0\% & - & - & - & - & - & - & - & - & - \\

% \hline
% Null Pointer Dereference Prevention Checklist & 4 & 0\% & 25\% & 10 & 20\% & 20\% & 25 & 12\% & 16\% & 79 & 4\% & 18\% & 123 & 7\% & 17\% & 202 & 5\% & 17\% \\

% \hline
%     \end{tabularx}
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{RQ2 - Type automatically generated }
%     \label{tab:rq2type}
%     \begin{tabularx}{\textwidth}{p{8cm}|rXX|rXX}
%     \hline
%          & \multicolumn{3}{c|}{\textbf{Open-source}}& \multicolumn{3}{c}{\textbf{Closed-source}} \\
         
%         &Tot&Acc&App&Tot&Acc&App\\
%          \hline


% \textbf{CLUSTER K=5}\\\hline
% Code Readability and Maintainability Improvements & 20 ( 6\%) & 15\% & 20\% & 162 (14\%) & 10\% & 24\% \\
% \hline
% Code Refactoring and Error Handling Enhancements & 80 (24\%) & 2\% & 2\% & 8 ( 1\%) & 0\% & 0\% \\
% \hline
% Code Review Feedback and Recommendations & 178 (53\%) & 11\% & 16\% & 210 (18\%) & 11\% & 29\% \\
% \hline
% Code Review and Validation Checklist & 11 ( 3\%) & 0\% & 0\% & 309 (26\%) & 5\% & 34\% \\
% \hline
% Null Pointer Dereference and Error Handling Improvements & 48 (14\%) & 8\% & 12\% & 496 (42\%) & 6\% & 26\% \\
% \hline

% \textbf{CLUSTER K=8}\\\hline
% Code Quality and Error Handling Improvements & 144 (43\%) & 6\% & 8\% & 42 ( 4\%) & 12\% & 24\% \\
% \hline
% Code Quality and Maintenance Improvements & 82 (24\%) & 20\% & 23\% & 156 (13\%) & 17\% & 28\% \\
% \hline
% Code Readability and Maintainability Improvements & 13 ( 4\%) & 8\% & 15\% & 108 ( 9\%) & 8\% & 20\% \\
% \hline
% Code Review and Optimization Checklist & 20 ( 6\%) & 0\% & 5\% & 196 (17\%) & 6\% & 32\% \\
% \hline
% Code Review and Validation Checklist & 9 ( 3\%) & 0\% & 0\% & 182 (15\%) & 6\% & 35\% \\
% \hline
% Code Review and Validation Checklist for Game Development & 2 ( 1\%) & 0\% & 0\% & 206 (17\%) & 4\% & 37\% \\
% \hline
% Codebase Update and Refactoring Checklist & 45 (13\%) & 0\% & 2\% & 83 ( 7\%) & 1\% & 23\% \\
% \hline
% Null Pointer Dereference Risk Mitigations & 22 ( 7\%) & 18\% & 23\% & 212 (18\%) & 6\% & 18\% \\

% \hline
%     \end{tabularx}
% \end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{RQ2 - Type automatically generated }
%     \label{tab:rq2type}
%     \begin{tabularx}{\textwidth}{p{8cm}|rXX|rXX}
%     \hline
%          & \multicolumn{3}{c|}{\textbf{Open-source}}& \multicolumn{3}{c}{\textbf{Closed-source}} \\
         
%         &Total&Acceptance&Appreciation&Total&Acceptance&Appreciation\\
%          \hline


% \textbf{CLUSTER K=50}\\\hline
% Functional - Conditional Compilation & 3 ( 1\%) & 33\% & 33\% & 33 ( 3\%) & 3\% & 15\% \\
% \hline
% Functional - Initialization & 10 ( 3\%) & 0\% & 10\% & 41 ( 3\%) & 17\% & 49\% \\
% \hline
% Functional - Interface & 41 (12\%) & 10\% & 12\% & 74 ( 6\%) & 1\% & 27\% \\
% \hline
% Functional - Lambda Usage & 5 ( 1\%) & 0\% & 20\% & 17 ( 1\%) & 0\% & 29\% \\
% \hline
% Functional - Logging/Error Handling & 5 ( 1\%) & 0\% & 0\% & 37 ( 3\%) & 14\% & 38\% \\
% \hline
% Functional - Logical & 100 (28\%) & 7\% & 14\% & 229 (19\%) & 6\% & 32\% \\
% \hline
% Functional - Resource & 34 (10\%) & 0\% & 0\% & 1 ( 0\%) & 0\% & 0\% \\
% \hline
% Functional - Timing & 2 ( 1\%) & 0\% & 0\% & 60 ( 5\%) & 3\% & 27\% \\
% \hline
% Functional - Validation & 109 (31\%) & 13\% & 21\% & 526 (44\%) & 7\% & 25\% \\
% \hline
% Refactoring - Code Quality and Consistency & 9 ( 3\%) & 22\% & 33\% & 26 ( 2\%) & 15\% & 38\% \\
% \hline
% Refactoring - Include Management & 2 ( 1\%) & 0\% & 0\% & 23 ( 2\%) & 26\% & 48\% \\
% \hline
% Refactoring - Organization of the code & 19 ( 5\%) & 16\% & 16\% & 24 ( 2\%) & 8\% & 33\% \\
% \hline
% Refactoring - Readability and Maintainability & 6 ( 2\%) & 0\% & 17\% & 31 ( 3\%) & 6\% & 16\% \\
% \hline
% Refactoring - Simplification & 8 ( 2\%) & 12\% & 25\% & 61 ( 5\%) & 8\% & 20\% \\
% \hline
% Refactoring - Visual Representation & 2 ( 1\%) & 0\% & 0\% & 2 ( 0\%) & 50\% & 50\% \\

% \hline
% \textbf{CLUSTER K=50 simplified}\\
% \hline
% Functional & 309 (87\%) & 8\% & 15\% & 1018 (86\%) & 6\% & 28\% \\
% \hline
% Refactoring & 46 (13\%) & 13\% & 20\% & 167 (14\%) & 12\% & 28\% \\
    
    
%     \end{tabularx}
% \end{table*}

% \begin{table}[t]
%     \centering
%     \caption{RQ2 - For each automatically generated comment category, the number of comments labelled as such are shown for Organization1 and 2.}
%     \label{tab:clusteragg}
%     \begin{tabularx}{\linewidth}{l||Xr|Xr|Xr|Xr}
%     \hline
%          Label& \multicolumn{4}{c|}{\textbf{Organization1}}& \multicolumn{4}{c}{\textbf{Organization2}} \\
%          \hline
%         &\multicolumn{2}{c|}{\textbf{Code}}& \multicolumn{2}{c|}{\textbf{Ex}}&\multicolumn{2}{c|}{\textbf{Code}}& \multicolumn{2}{c}{\textbf{Ex}}\\
%         \hline

% % Functional & 132 ; 82.5\% & 253 (79.6\%) & 490 (84.5\%) & 500 (82.6\%) \\
% % Refactoring & 28 (17.5\%) & 50 (15.7\%) & 83 (14.3\%) & 98 (16.2\%) \\
% % Documenta. & 0 ( 0\%) & 9 (2.8\%) & 5 (0.9\%) & 2 (0.3\%) \\
% % Discussion & 0 ( 0\%) & 6 (1.9\%) & 2 (0.3\%) & 5 (0.8\%) \\
% % Functional & 132 - 82.5\% & 253 - 79.6\% & 490 - 84.5\% & 500 - 82.6\% \\
% % Refactoring & 28 - 17.5\% & 50 - 15.7\% & 83 - 14.3\% & 98 - 16.2\% \\
% % Documentat. & 0 - 0\% & 9 2.8\% & 5 - 0.9\% & 2 - 0.3\% \\
% % Discussion & 0 - 0\% & 6 - 1.9\% & 2 - 0.3\% & 5 - 0.8\% \\
% Functional & 97 & 76.4\% & 234 & 80.4\% & 500 & 86.2\% & 505 & 83.5\% \\
% Refactoring & 26 & 20.5\% & 40 & 13.7\% & 77 & 13.3\% & 95 & 15.7\% \\
% Documentation & 3 & 2.4\% & 8 & 2.7\% & 3 & 0.5\% & 1 & 0.2\% \\
% Discussion & 1 & 0.8\% & 9 & 3.1\% & 0& 0\% & 4 & 0.7\% \\
% % \hline
% % Total& 127 && 291 && 580 && 605 &  \\

% \hline
%     \end{tabularx}
% \end{table}


\begin{table}[t]
    \centering
    \caption{RQ2 - For each automatically generated comment category, we list the number of comments from each Organization (Moz and Ubi) that were labeled as such.``*" indicates that the label was an example in the few-shot prompt~\cite{turzo2024makes}. }
    \label{tab:cluster}
    \begin{tabularx}{\linewidth}{c|l|X|X}
    \hline
         \#&Label& \textbf{Moz.}& \textbf{Ubi.} \\
         \hline

1 & Discussion - Design discussion * & 3  & 3  \\
2 & Discussion - Question * & 7  & 1  \\
3 & Documentation * & 11  & 4  \\
4 & Functional - Conditional Compilation & 2  & 11  \\
5 & Functional - Consistency and Thread Safety & 1  & 0 \\
6 & Functional - Error Handling & 4  & 2  \\
7 & Functional - Exception Handling & 0 & 2  \\
8 & Functional - Initialization & 1  & 8  \\
9 & Functional - Interface *& 81  & 91  \\
10 & Functional - Lambda Usage & 2  & 3  \\
11 & Functional - Logical *& 74  & 272  \\
12 & Functional - Null Handling & 0 & 3  \\
13 & Functional - Performance & 3  & 18  \\
14 & Functional - Performance Optimization & 0 & 1  \\
15 & Functional - Performance and Safety & 0 & 1  \\
16 & Functional - Resource * & 58  & 135  \\
17 & Functional - Security & 1  & 0 \\
18 & Functional - Serialization & 0 & 4  \\
19 & Functional - Support * & 3  & 2  \\
20 & Functional - Syntax & 3  & 2  \\
21 & Functional - Timing * & 3  & 56  \\
22 & Functional - Type Safety & 0 & 2  \\
23 & Functional - Validation *& 95  & 392  \\
24 & Refactoring - Alternate Output * & 11  & 6  \\
25 & Refactoring - Code Duplication & 0 & 7  \\
26 & Refactoring - Code Simplification & 0 & 2  \\
27 & Refactoring - Consistency & 0 & 1  \\
28 & Refactoring - Magic Numbers & 0 & 1  \\
29 & Refactoring - Naming Convention * & 15  & 24  \\
30 & Refactoring - Organization of the code * & 10  & 79  \\
31 & Refactoring - Performance Optimization & 0 & 6  \\
32 & Refactoring - Readability & 3  & 11  \\
33 & Refactoring - Simplification & 0 & 3  \\
34 & Refactoring - Solution approach * & 26  & 27  \\
35 & Refactoring - Unused Variables & 0 & 1  \\
36 & Refactoring - Variable Declarations & 0 & 1  \\
37 & Refactoring - Visual Representation & 1  & 3  \\        
\hline
    \end{tabularx}
\end{table}



% \begin{table}[t]
%     \centering
%     \caption{RQ2 - Categorization of generated comment and associated appreciation and acceptance.}
%     \label{tab:clusteragg}
%     \begin{tabularx}{\linewidth}{l||rr|X|X||rr|X|X}
%     \hline
%          Categories& \multicolumn{4}{c|}{\textbf{Mozilla}}& \multicolumn{4}{c}{\textbf{Ubisoft}} \\
%          \hline
%         &\multicolumn{2}{c|}{\textbf{Total}}&\textbf{Acc}&\textbf{App}&\multicolumn{2}{c|}{\textbf{Total}}&\textbf{Acc}&\textbf{App}\\
%         &[\#]&[\%]&[\%]&[\%]&[\#]&[\%]&[\%]&[\%]\\
%         \hline

% % Functional & 132 ; 82.5\% & 253 (79.6\%) & 490 (84.5\%) & 500 (82.6\%) \\
% % Refactoring & 28 (17.5\%) & 50 (15.7\%) & 83 (14.3\%) & 98 (16.2\%) \\
% % Documenta. & 0 ( 0\%) & 9 (2.8\%) & 5 (0.9\%) & 2 (0.3\%) \\
% % Discussion & 0 ( 0\%) & 6 (1.9\%) & 2 (0.3\%) & 5 (0.8\%) \\
% % Functional & 132 - 82.5\% & 253 - 79.6\% & 490 - 84.5\% & 500 - 82.6\% \\
% % Refactoring & 28 - 17.5\% & 50 - 15.7\% & 83 - 14.3\% & 98 - 16.2\% \\
% % Documentat. & 0 - 0\% & 9 2.8\% & 5 - 0.9\% & 2 - 0.3\% \\
% % Discussion & 0 - 0\% & 6 - 1.9\% & 2 - 0.3\% & 5 - 0.8\% \\
% Functional & 331 & 79.2 &4.8&19.0&1005& 84.8&5.2 &29.0\\
% Refactoring & 66 &15.8 &18.2&36.4& 172&14.5&18.6&25.0\\
% Documentation & 11 &2.6 &-&-& 4 &.34 &-&- \\
% Discussion & 10 &2.4 &-&-& 4&.34 &-&-\\
% % \hline
% % Total& 127 && 291 && 580 && 605 &  \\

% \hline
%     \end{tabularx}
% \end{table}


\begin{table}[t]
    \centering
    \caption{RQ2 - Categorization of generated comment and associated appreciation and acceptance.}
    \label{tab:categoryres}
    \begin{tabularx}{.99\linewidth}{l|XXXX|XXXX}
    \hline
        \textbf{Organization} & \multicolumn{4}{c|}{\textbf{Mozilla}}& \multicolumn{4}{c}{\textbf{Ubisoft}} \\
         \hline
    \diagbox[dir=NW, width=2.5cm, height=2cm]{\textbf{Metric}}{\textbf{Category}}&\rotatebox[origin=c]{75}{\textbf{Functional}}
    &\rotatebox[origin=c]{75}{\textbf{Refactoring}}
    &\rotatebox[origin=c]{75}{\textbf{Documentation}}
    &\rotatebox[origin=c]{75}{\textbf{Discussion}}
    &\rotatebox[origin=c]{75}{\textbf{Functional}}
    &\rotatebox[origin=c]{75}{\textbf{Refactoring}}
    &\rotatebox[origin=c]{75}{\textbf{Documentation}}
    &\rotatebox[origin=c]{75}{\textbf{Discussion}}\\
        % &Functi-onal&Refac-tor- ing&Docu-men-tation&Discu-ssion&Functi-onal&Refac-toring&Docu-men-tation&Discu-ssion\\
        % &\multicolumn{2}{c|}{\textbf{Total}}&\textbf{Acc}&\textbf{App}&\multicolumn{2}{c|}{\textbf{Total}}&\textbf{Acc}&\textbf{App}\\
        % &[\#]&[\%]&[\%]&[\%]&[\#]&[\%]&[\%]&[\%]\\
        \hline
        Count [\#]&331&66&11&10&1005&172&4&4\\
        \hline
        \%Total [\%]&79.2&15.8&2.6&2.4&84.8&14.5&.34&.34\\
        Acceptance [\%]&4.8&18.2&-&-&5.2&18.6&-&-\\
        Appreciation [\%]&19.0&36.4&-&-&29.0&25.0&-&-\\

% Functional & 132 ; 82.5\% & 253 (79.6\%) & 490 (84.5\%) & 500 (82.6\%) \\
% Refactoring & 28 (17.5\%) & 50 (15.7\%) & 83 (14.3\%) & 98 (16.2\%) \\
% Documenta. & 0 ( 0\%) & 9 (2.8\%) & 5 (0.9\%) & 2 (0.3\%) \\
% Discussion & 0 ( 0\%) & 6 (1.9\%) & 2 (0.3\%) & 5 (0.8\%) \\
% Functional & 132 - 82.5\% & 253 - 79.6\% & 490 - 84.5\% & 500 - 82.6\% \\
% Refactoring & 28 - 17.5\% & 50 - 15.7\% & 83 - 14.3\% & 98 - 16.2\% \\
% Documentat. & 0 - 0\% & 9 2.8\% & 5 - 0.9\% & 2 - 0.3\% \\
% Discussion & 0 - 0\% & 6 - 1.9\% & 2 - 0.3\% & 5 - 0.8\% \\
% Functional & 331 & 79.2 &4.8&19.0&1005& 84.8&5.2 &29.0\\
% Refactoring & 66 &15.8 &18.2&36.4& 172&14.5&18.6&25.0\\
% Documentation & 11 &2.6 &-&-& 4 &.34 &-&- \\
% Discussion & 10 &2.4 &-&-& 4&.34 &-&-\\
% \hline
% Total& 127 && 291 && 580 && 605 &  \\

\hline
    \end{tabularx}
\end{table}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq4_impact.tex <==

\begin{table}[t]
    \centering
    \caption{RQ4 - Impact of generated comments on finished patch reviews. ``Generated" refers to accepted generated comment. ``Human" refers to manually written comments on patches without generated comments.}
    \label{tab:rq4res}
    \begin{tabularx}{\linewidth}{r|Xr|Xr}
    \hline
         \textbf{Evaluation}& \multicolumn{4}{c}{\textbf{Ubisoft}} \\
         & \multicolumn{2}{c|}{\textbf{Generated}}& \multicolumn{2}{c}{\textbf{Human}} \\
         \hline

Revised line & 43 &62.3\% & 779 &64.3\% \\
Revised hunk & 51 &73.9\% & 887 &73.2\% \\
Thread  & 16 &23.2\% & 411 &33.9\% \\
\hline Total  & 69 && 1211 \\
\hline
    \end{tabularx}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{RQ4 - Impact of generated comments on finished patch reviews. "Generated" refers to accepted generated comment. "Human" refers to manually written comments on patches without generated comments.}
%     \label{tab:rq4res}
%     \begin{tabularx}{\linewidth}{r|Xr|Xr|Xr|Xr}
%     \hline
%          \textbf{Evaluation}& \multicolumn{4}{c|}{\textbf{Company1}}& \multicolumn{4}{c}{\textbf{Company2}} \\
%          & \multicolumn{2}{c|}{\textbf{Generated}}& \multicolumn{2}{c|}{\textbf{Human}}& \multicolumn{2}{c|}{\textbf{Generated}}& \multicolumn{2}{c}{\textbf{Human}} \\
%          \hline


% Revised line & 7&28.\% & -&- & 43 &62.3\% & 779 &64.3\% \\
% Revised hunk & 14&56.\% & -&- & 51 &73.9\% & 887 &73.2\% \\
% Thread  & 5&20.\% & -&- & 16 &23.2\% & 411 &33.9\% \\
% \hline Total & 25& & -&- & 69 && 1211 \\
% \hline
% % \hline


%     \end{tabularx}
% \end{table}
% \begin{table}[t]
%     \centering
%     \caption{RQ4 - Impact of generated comments on finished patch reviews. "Generated" refers to accepted generated comment. "Human" refers to manually written comments on patches without generated comments.}
%     \label{tab:rq4res}
%     \begin{tabularx}{\linewidth}{r|c|Xr|Xr}
%     \hline
%          \textbf{Evaluation}& \multicolumn{1}{c|}{\textbf{Organization1}}& \multicolumn{4}{c}{\textbf{Organization2}} \\
%          & \multicolumn{1}{c|}{\textbf{Generated}}& \multicolumn{2}{c|}{\textbf{Generated}}& \multicolumn{2}{c}{\textbf{Human}} \\
%          \hline


% Revised line & 7& 43 &62.3\% & 779 &64.3\% \\
% Revised hunk & 14 & 51 &73.9\% & 887 &73.2\% \\
% Thread  & 5 & 16 &23.2\% & 411 &33.9\% \\
% \hline Total & 25 & 69 && 1211 \\
% \hline
% % \hline


%     \end{tabularx}
% \end{table}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/rq5_edits.tex <==

\begin{table}[t]
    \centering
    \caption{RQ3 - Editing of accepted comments}
    \label{tab:edits}
    \begin{tabularx}{\linewidth}{l|X|X}
    \hline
         \textbf{Evaluation}& \multicolumn{1}{c|}{\textbf{Organization1}}& \multicolumn{1}{c}{\textbf{Organization2}} \\
         % &\textbf{Code}&\textbf{Example}&\textbf{Code}&\textbf{Example}\\
         \hline
         % \hline
Suggestion as-is&    27  & 55\\
Shortened content&    6 & 19\\
Additional content&  1  & 4\\
Other modification&  0 & 7\\
% \hline
% Moved suggestion&    &\\
         \hline 
    \end{tabularx}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{RQ5 - Edition on accepted comments \Do{probably not showing by approach but total of generated comments}}
%     \label{tab:edits}
%     \begin{tabularx}{\linewidth}{l|X|X|X|X}
%     \hline
%          \textbf{Evaluation}& \multicolumn{2}{c|}{\textbf{Open-source}}& \multicolumn{2}{c}{\textbf{Closed-source}} \\
%          &\textbf{Code}&\textbf{Example}&\textbf{Code}&\textbf{Example}\\
%          \hline\hline
% Suggestion as-is&   &   & 14  & 34\\
% Additional content&   &   & 3  & 1\\
% Shortened content&   &   &  2 & 11\\
% Other modification&   &   & 2  & 3\\
% \hline
% Moved suggestion&   &   &   &\\
%          \hline 
%     \end{tabularx}
% \end{table}


==> zkbqmyqdxhpftbqxtqyyrmfmgfjnnhdw/tables/survey.tex <==
\begin{table}[t]
    \centering
    \caption{End of study survey questions}
    \label{tab:survey}
    \begin{tabularx}{\linewidth}{|l|X|}
    \hline
       \#& \textbf{Question} \\
    \hline
    1&What is your experience as a developer in the company? (in years)\\\hline
    2&What is your experience as a developer in your carreer? (in years)\\\hline
    % 3&Do you find the tool's suggestions distracting during your reviews?\newline
    % Never - Rarely - Sometimes - Often - Always
    % \\\hline
    3&When using the tool, how was the duration of your reviews affected? \newline
    Slower - A bit slower - Same time - A bit quicker - Quicker
    \\\hline
    % 5&In most cases, what do you think about the quantity of suggestions? \newline 
    % Always not enough - Sometimes not enough - Moderate number - Sometimes too many - Always too many
    % \\\hline
    4&What would you change about the generated comments' content, if anything? (open) \\\hline
    % 5&What would you change about the way suggestions are shown, if anything? (open)\\\hline
    5&Would you use a review tool like this tool during your review processes outside of the study? \newline 
    Never - Rarely - Sometimes - Often - Always\\\hline
    % 9&What is your position regarding the use of generative AI in code development and code review? \newline
    % Totally opposed - Partially opposed - Neutral - Partially favorable - Totally favorable\\\hline
    % 10&Did your view on Generative AI for code development and code review change after this study? (open)\\\hline
    \end{tabularx}
\end{table}
